Marlin: Efficient Coordination for Autoscaling Cloud DBMS (Extended Version)

Modern cloud databases are shifting from converged architectures to storage disaggregation, enabling independent scaling and billing of compute and storage. However, cloud databases still rely on external, converged coordination services (e.g., ZooKeeper) for their control planes. These services are effectively lightweight databases optimized for low-volume metadata. As the control plane scales in the cloud, this approach faces similar limitations as converged databases did before storage disaggregation: scalability bottlenecks, low cost efficiency, and increased operational burden. We propose to disaggregate the cluster coordination to achieve the same benefits that storage disaggregation brought to modern cloud DBMSs. We present Marlin, a cloud-native coordination mechanism that fully embraces storage disaggregation. Marlin eliminates the need for external coordination services by consolidating coordination functionality into the existing cloud-native database it manages. To achieve failover without an external coordination service, Marlin allows cross-node modifications on coordination states. To ensure data consistency, Marlin employs transactions to manage both coordination and application states and introduces MarlinCommit, an optimized commit protocol that ensures strong transactional guarantees even under cross-node modifications. Our evaluations demonstrate that Marlin improves cost efficiency by up to 4.4x and reduces reconfiguration duration by up to 4.9x compared to converged coordination solutions.

==> figures/plots_code/1_intro/f1.tex <==
\begin{figure}
    \centering
    \begin{adjustbox}{width=\columnwidth,center}
        
    \begin{tabular}{@{}c@{\hspace{0.02\linewidth}}c@{}}
        \begin{tikzpicture}[scale=0.5]
            % Axes
            \draw[->] (0,0) -- (6,0) node[right] {dynamicity};
            \draw[->] (0,0) -- (0,4) node[above] {Latency};
            
            % Curves
            \draw[thick, color={rgb,255:red,255; green,165; blue,0}] (0,0.7) -- (6,0.7);
            \draw[thick, color={rgb,255:red,70; green,130; blue,180}] (0,0.7) .. controls (5,0.7) .. (5.1,3.4);
            \draw[thick, color={rgb,255:red,128; green,0; blue,128}] (0,0.7) .. controls (2.5,0.7) and (2.8,0.7) .. (3,3.4);
            % Labels
            \node[above right] at (1.5,3.5) {Small ZK};
            \node[above right] at (3.5,3.5) {Large ZK};
            \node[right] at (6,0.3) {Marlin};

        \end{tikzpicture}
        &
        \begin{tikzpicture}[scale=0.5]
            % Axes
            \draw[->] (0,0) -- (6,0) node[right] {dynamicity};
            \draw[->] (0,0) -- (0,4) node[above] {Cost};
            
            % Curves
            \draw[thick, color={rgb,255:red,70; green,130; blue,180}, name path=C] (0,2) .. controls (4,2.1) and (5,2.5) .. (6,5);
            \draw[thick, color={rgb,255:red,128; green,0; blue,128}, name path=D] (0,1.3) .. controls (2,1.5) and (3,1.8) .. (4,4);
            \draw[thick, color={rgb,255:red,255; green,165; blue,0}] (0,0.7) -- (6,0.7);
            \draw[dashed] (0,0.4) -- (6,0.4);
            % \addplot[green!20] fill between[of=C and D];
            % \fill[blue!20, opacity=0.5] (0,1.3) -- plot[name path=C] coordinates {(0,2) .. controls (4,2.1) and (5,2.5) .. (6,5)}
            % -- plot[name path=D] coordinates {(0,1.3) .. controls (2,1.5) and (3,1.8) .. (4,4)} -- cycle;

            \node[draw, circle, inner sep=1pt, fill=white] at (1, 1.7) {1};
            \node[draw, circle, inner sep=1pt, fill=white] at (4.5, 3.3) {2};

            % Labels
            \node[above right] at (2,3.5) {Small ZK};
            \node[above right] at (4,3.5) {Large ZK};
            \node[right] at (6,0.7) {Marlin};
            \node[right] at (6,0.3) {perfect system};
        \end{tikzpicture}
        \\
        (a) Latency & (b) Cost
    \end{tabular}
    \end{adjustbox}
    \caption{\textbf{Scalability and Cost Over Workload Dynamicity}}
    \label{fig:intro_f1}
\end{figure}



==> figures/plots_code/1_intro/f1_back.tex <==

\begin{figure}
    % \centering
	\begin{subfigure}{0.5\columnwidth}%
    	\centering
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev1-cost-breakdown.png}  
        \caption{Scalability Issue}
        \label{fig:intro_f1_a}
    \end{subfigure}%
    % \par\medskip
    \hfill
    \begin{subfigure}{0.5\columnwidth}%
    	\centering
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev1-migr-latency-breakdown.png}  
        \caption{Cost Issue}
        \label{fig:intro_f1_b}
    \end{subfigure}%
    % \vspace{-.15in}
    % \setlength{\belowcaptionskip}{-10pt}
    \caption{\textbf{Zookeeper's Scalability and Cost Issues}}
    \label{fig:intro_f1}
\end{figure}



% \begin{figure*}[t]
% 	% \begin{subfigure}[b]{0.48\linewidth}%
%         % \centering
%         \begin{subfigure}[b]{0.25\linewidth}%
%             \center
%             % \captionsetup{justification=centering}
%             % \includegraphics[width=.8\linewidth]{figures/backgrounds/fig1.jpg}
%             \includegraphics[width=\linewidth]{figures/plots/2_moti/2_moti_f1_a.pdf}     
%             \caption{Scalability Issue}
%             \label{fig:moti_f1_a}
%         \end{subfigure}%
%     \begin{subfigure}[b]{0.25\linewidth}%
%     	\center
%         % \captionsetup{justification=centering}
%         \includegraphics[width=\linewidth]{figures/plots/2_moti/2_moti_f1_c.pdf}         
%         \caption{Cost Issue}
%         \label{fig:moti_f1_c}
%     \end{subfigure}%

%     \vspace{-.1in}
%     % \setlength{\belowcaptionskip}{-10pt}
%     \caption{\textbf{Zookeeper's Scalability and Cost Issues}}
%     % \caption{\textbf{Disaggregated DBMS Architectures} --- \normalfont{The green parts represent the management of system states.}
%     %The control plane is not shown for simplicity.}
%     %\yxy{a few extra suggestions: (1) the nodes can be narrower (if need space). (2) the green part in Figure 1(a) can look a little different from the other parts; right now it looks a bit like the system state is a third partition of the cluster.}
%     %\wjh{cannot find a good way to represent auxiliary service. Any concrete suggestions? Also I think it can be better to keep three figures.}\yxy{The current solution looks good to me. If we keep 3 figures, where do we discuss the middle one? }
    
%     \label{fig:moti_f1}
% \end{figure*}

==> figures/plots_code/2_motivation/ServiceDowntimeBreakdown.tex <==
\begin{table*}[th]
    \begin{center}
            % \setlength{\belowcaptionskip}{-10pt}
    \caption{Service Downtime Breakdown Analysis}
    \label{tbl:moti_downtime_breakdown}
    \vspace{-3mm}
    \small
    \begin{tabular}{ l l l l l l }
    \toprule
    \multicolumn{1}{c}{} &\multicolumn{5}{c}{\textbf{Push Reconfiguration}} \\
    \cline{2-6} 
    \textbf{Indicators} & \textcolor{red}{\textbf{\system(Hybrid-Heat)}} & \textbf{Lock \& Abort} & \textcolor{red}{\textbf{Albatross}} & \textbf{DynaMast} & \textbf{Remus} \\ 
    \midrule
    % Wait for On-going Txn & \makecell{Yes\\(only for conflicted txns)} & No & No & Yes(for all on-going txns) & No && Yes(only for conflicted txns) & No\\
    Wait for On-going Txn & Yes (for conflicted txns) & No & No & Yes (for all on-going txns) & No\\
    Flush Updates in Src Node & No & Yes & Yes & Yes & No \\
    Copy Remaining State & No & Yes & Yes & Yes & No\\
    Copy Txn State & No & No & Yes & No & No\\
    % Ownership Transfer & Yes & Yes & Yes & Yes & Yes && Yes & Yes\\
    

    \bottomrule
    \end{tabular}
    \end{center}
    \end{table*}

==> figures/plots_code/2_motivation/f1_alternative.tex <==
\begin{figure*}[t]
    \centering
    % First subfigure
    \begin{subfigure}[b]{0.28\linewidth}
        \centering
        \begin{tikzpicture}
            % Storage
            \node (storage) [draw, rectangle, minimum width=3cm, minimum height=1cm] {Storage};
            % Nodes
            \node (rNode1) [draw, rectangle, above=1cm of storage, minimum width=1cm] {R Node};
            \node (rwNode) [draw, rectangle, left=0.5cm of rNode1, minimum width=1cm] {RW Node};
            \node (rNode2) [draw, rectangle, right=0.5cm of rNode1, minimum width=1cm] {R Node};
            % Arrows
            \draw[<->] (rwNode) -- (storage);
            \draw[<-] (rNode1) -- (storage);
            \draw[<-] (rNode2) -- (storage);
        \end{tikzpicture}
        \caption{Single-Writer}
        \label{fig:moti_f1_a}
    \end{subfigure}
    \hspace{0.1cm}  % Reduced horizontal space
    % Second subfigure
    \begin{subfigure}[b]{0.28\linewidth}
        \centering
        \begin{tikzpicture}
            \node [draw, rectangle, minimum width=1cm, minimum height=1.6cm, text height=0.05cm, text depth=0.1cm] (rw1) {RW Node};
            \node [draw, rectangle, right=0.2cm of rw1, minimum width=1cm, minimum height=1.6cm, text height=0.05cm, text depth=0.1cm] (rw2) {RW Node};
            \node [draw, rectangle, right=0.2cm of rw2, minimum width=1cm, minimum height=1.6cm, text height=0.05cm, text depth=0.1cm] (rw3) {RW Node};
            \node [draw, rectangle, below=0.5cm of rw2, minimum width=3cm, minimum height=1cm] (storage) {Storage};
            \node [draw, dashed, rectangle, fill=white, fill opacity=1, above=0.6cm of storage, minimum width=5cm, minimum height=0.5cm] (protocol) {Coherent Cache Protocol};
            % \node [above=0.1cm of protocol] {Coherent Cache Protocol};

            \draw[<->] (storage) -- (rw1);
            \draw[<->] (storage) -- (rw2);
            \draw[<->] (storage) -- (rw3);
        \end{tikzpicture}
        \caption{Shared-Writer}
        \label{fig:moti_f1_b}
    \end{subfigure}
    \hspace{0.1cm}  % Reduced horizontal space
    % Third subfigure
    \begin{subfigure}[b]{0.28\linewidth}
        \centering
        \begin{tikzpicture}
            % Storage Partitions
            \node (partition2) [draw, rectangle, minimum width=0.6cm, minimum height=1cm] {Partition 2};
            \node (partition1) [draw, rectangle,left=0.2cm of partition2,  minimum width=0.6cm, minimum height=1cm] {Partition 1};
            \node (partition3) [draw, rectangle, right=0.2cm of partition2, minimum width=0.6cm, minimum height=1cm] {Partition 3};
            \node (storage) [draw, rectangle, minimum width=5.5cm, minimum height=1.7cm, anchor=center, yshift=0.2cm] at (partition2) {\raisebox{1.1cm}{Storage}};
            % Nodes
            \node (rwNode1) [draw, rectangle, above=1cm of partition1, minimum width=1cm] {RW Node};
            \node (rwNode2) [draw, rectangle, above=1cm of partition2, minimum width=1cm] {RW Node};
            \node (rwNode3) [draw, rectangle, above=1cm of partition3, minimum width=1cm] {RW Node};
            % Arrows
            \draw[<->] (rwNode1) -- (partition1);
            \draw[<->] (rwNode2) -- (partition2);
            \draw[<->] (rwNode3) -- (partition3);
        \end{tikzpicture}
        \caption{Partitioned-Writer}
        \label{fig:moti_f1_c}
    \end{subfigure}
    \caption{Diagrams of three architecture choices for Cloud OLTP Databases}
    \label{fig:moti_f1}
\end{figure*}

==> figures/plots_code/2_motivation/f2_back.tex <==
\begin{figure*}[t]
	% \begin{subfigure}[b]{0.48\linewidth}%
        \centering
        \begin{subfigure}[b]{0.5\linewidth}%
            \center
            % \captionsetup{justification=centering}
            % \includegraphics[width=.8\linewidth]{figures/backgrounds/fig1.jpg}
            \includegraphics[width=\linewidth]{figures/plots/2_moti/2_moti_f1_a.pdf}     
            \caption{Separation of Application and System States}
            \label{fig:moti_f2_a}
        \end{subfigure}%
    \begin{subfigure}[b]{0.5\linewidth}%
    	\center
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/2_moti/2_moti_f1_c.pdf}         
        \caption{Unified Storage on Storage Disaggregation}
        \label{fig:moti_f2_c}
    \end{subfigure}%

    \vspace{-.1in}
    % \setlength{\belowcaptionskip}{-10pt}
    \caption{\textbf{Disaggregated DBMS Architectures} --- \normalfont{The green parts represent the management of system states.}
    %The control plane is not shown for simplicity.}
    %\yxy{a few extra suggestions: (1) the nodes can be narrower (if need space). (2) the green part in Figure 1(a) can look a little different from the other parts; right now it looks a bit like the system state is a third partition of the cluster.}
    %\wjh{cannot find a good way to represent auxiliary service. Any concrete suggestions? Also I think it can be better to keep three figures.}\yxy{The current solution looks good to me. If we keep 3 figures, where do we discuss the middle one? }
    }
    \label{fig:moti_f2}
\end{figure*}



% \begin{figure*}[t]
% 	% \begin{subfigure}[b]{0.48\linewidth}%
%         \centering
%     % \begin{subfigure}[t]{0.5\columnwidth}%h
%     % 	\center
%     %     \captionsetup{justification=centering}
%     %     % \includegraphics[width=\linewidth]{figures/plots/experiment/ev-1-usertxn-latency.pdf}        
%     %     \includegraphics[width=\linewidth]{figures/plots/motivation/2_moti_nothing_zk.png}        
%     %  \caption{Segragated Storage on Shared-Nothing}
%     %     \label{fig:lw_migr_user_throughput}
%     % \end{subfigure}%
%     \begin{subfigure}[b]{0.5\linewidth}%
%     	\center
%         \captionsetup{justification=centering}
%         % \includegraphics[width=\linewidth]{figures/plots/experiment/ev-1-usertxn-latency.pdf}        
%         \includegraphics[width=\columnwidth]{figures/plots/2_moti/2_moti_f1_a.pdf}        

%      \caption{Segragated Storage on Shared-Nothing}
%         \label{fig:moti_f1_a}
%     \end{subfigure}%
%     % \vspace{.3in}
%     % \begin{subfigure}[t]{0.8\columnwidth}%
%     % 	\center
%     %     \captionsetup{justification=centering}
%     %     \includegraphics[width=\linewidth]{figures/plots/2_moti/2_moti_f1_b.pdf}        

%     %  \caption{Segragated Storage on Storage Disaggregation}
%     %     \label{fig:moti_f1_b}
%     % \end{subfigure}%
%     % \vspace{.3in}
%     \begin{subfigure}[b]{0.5\linewidth}%
%     	\center
%         \captionsetup{justification=centering}
%         \includegraphics[width=\columnwidth]{figures/plots/2_moti/2_moti_f1_c.pdf}        

%      \caption{Unified Storage on Storage Disaggregation}
%         \label{fig:moti_f1_c}
%     \end{subfigure}%
%     % \vspace{-.15in}
%     % \setlength{\belowcaptionskip}{-10pt}
%     % \setlength{\abovecaptionskip}{-10pt}

%     \caption{\textbf{DBMS Architectures for Cluster Management} --- \normalfont{The green boxes are the auxiliary services. The control plane is not shown for simplicity.}
%     \yxy{a few extra suggestions: (1) the nodes can be narrower (if need space). (2) the green part in Figure 1(a) can look a little different from the other parts; right now it looks a bit like the system state is a third partition of the cluster.}
%     }
%     \label{fig:moti_f1}
% \end{figure*}




==> figures/plots_code/2_motivation/f2_new_back.tex <==
\begin{figure*}[t]
    \centering
    % First subfigure
    \begin{subfigure}[t]{0.6\textwidth}
        \centering
        \begin{tikzpicture}[scale=1]

    % \tikzset{boxarrow/.style={draw, thick, -{Stealth[length=8mm, width=5mm]}-{Stealth[length=8mm, width=5mm]}, line width=0.6mm}}

            \node [draw, dashed, rectangle, fill=white, fill opacity=0.5, minimum width=3cm, minimum height=3.5cm] (CoorRec) at (6, 3) {Coordinator};

            % Coordinator part
            \node[draw, rectangle, minimum width=1cm, minimum height=1.5cm] (coordinator) at (6, 4) {C1};
            \node[draw, rectangle, minimum width=1cm, minimum height=1.5cm] (c1) at (5, 2) {C2};
            \node[draw, rectangle, minimum width=1cm, minimum height=1.5cm] (c2) at (7, 2) {C3};
            
            % Curved arrows between the coordinator and C nodes
            \draw[<->, thick, bend right] (coordinator) to (c1);
            \draw[<->, thick, bend left] (coordinator) to (c2);
            \draw[<->, thick, bend right] (c1) to (c2);
             \node [draw, dashed, rectangle, fill=white, fill opacity=0.5, minimum width=4.5cm, minimum height=2cm] (StorageRec) at (1.5, 2) {\raisebox{1.5cm}{Storage}};
            % RW chain
            \node[draw, rectangle, minimum width=1cm, minimum height=1cm, fill=white, fill opacity=1] (rw1) at (0, 4) {RW};
            \draw[->, thick, yshift=30pt] (rw1) to (coordinator);

            \node[draw, rectangle, minimum width=1cm, minimum height=1cm, fill=white, fill opacity=1] (rw2) at (1.5, 4) {RW};
            % \path[yshift=1.1cm] \draw[->, thick] (rw2) to (coordinator);
             \draw[->, thick, yshift=1.1cm] (rw2) -- ([yshift=1cm]coordinator);


            \node[draw, rectangle, minimum width=1cm, minimum height=1cm, fill=white, fill opacity=1] (rw3) at (3, 4) {RW};
            \draw[->, thick] (rw3) to (coordinator);

            \node[draw, rectangle, minimum width=1cm, minimum height=1cm] (block1) at (0, 2) {};
            \node[draw, rectangle, minimum width=1cm, minimum height=1cm] (block2) at (1.5, 2) {};
            \node[draw, rectangle, minimum width=1cm, minimum height=1cm] (block3) at (3, 2) {};

            % Curved arrows between RW nodes
            \draw[<->, thick] (rw1) to (rw2);
            \draw[<->, thick] (rw2) to (rw3);
            
            % Straight arrows from RW to blocks and coordinator
            \draw[<->, line width=1mm, draw=gray, opacity=0.5] (rw1) -- (block1);
            \draw[<->, line width=1mm, draw=gray, opacity=0.5] (rw2) -- (block2);
            \draw[<->, line width=1mm, draw=gray, opacity=0.5] (rw3) -- (block3);

        \end{tikzpicture}
        \caption{Centralized Coordinator}
        \label{fig:moti_f2_a}
    \end{subfigure}
    \hspace{0.2cm}  % Reduced horizontal space  
    % Second subfigure
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \begin{tikzpicture}[scale=1]
   
            % RW chain
            \node[draw, rectangle, minimum width=1cm, minimum height=1cm, fill=white, fill opacity=1] (rw1) at (0, 4) {RW};
            % \draw[->, thick] (rw1) to (coordinator);

            \node[draw, rectangle, minimum width=1cm, minimum height=1cm, fill=white, fill opacity=1] (rw2) at (1.5, 4) {RW};
            % \draw[->, thick] (rw2) to (coordinator);

            \node[draw, rectangle, minimum width=1cm, minimum height=1cm, fill=white, fill opacity=1] (rw3) at (3, 4) {RW};
            % \draw[->, thick] (rw3) to (coordinator);

            \node[draw, rectangle, minimum width=1cm, minimum height=1cm] (block1) at (0, 2) {};
            \node[draw, rectangle, minimum width=1cm, minimum height=1cm] (block2) at (1.5, 2) {};
            \node[draw, rectangle, minimum width=1cm, minimum height=1cm] (block3) at (3, 2) {};

            % Curved arrows between RW nodes
            \draw[<->, thick] (rw1) to (rw2);
            \draw[<->, thick] (rw2) to (rw3);
            
            % Straight arrows from RW to blocks and coordinator
            \draw[<->, thick] (rw1) -- (block1);
            \draw[<->, thick] (rw2) -- (block2);
            \draw[<->, thick] (rw3) -- (block3);
        \end{tikzpicture}
        \caption{Marlin}
        \label{fig:moti_f2_b}
    \end{subfigure}
    \caption{Metadata Management in Partitioned-Writer Systems}
    \label{fig:moti_f2}
\end{figure*}

==> figures/plots_code/2_motivation/f3.tex <==
\begin{figure*}[t]
	% \begin{subfigure}[b]{0.48\linewidth}%
        \centering
        \begin{subfigure}[b]{0.5\linewidth}%
            \center
            % \captionsetup{justification=centering}
            % \includegraphics[width=.8\linewidth]{figures/backgrounds/fig1.jpg}
            \includegraphics[width=\linewidth]{figures/plots/2_moti/2_moti_f2_a.pdf}     
            \caption{Centralized Coordination Service}
            \label{fig:moti_f3_a}
        \end{subfigure}%
    \begin{subfigure}[b]{0.5\linewidth}%
    	\center
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/2_moti/2_moti_f2_b.pdf}         
        \caption{\system}
        \label{fig:moti_f3_b}
    \end{subfigure}%

    \vspace{-.1in}
    % \setlength{\belowcaptionskip}{-10pt}
    \caption{\textbf{Coordination Demonstration}.}

    \label{fig:moti_f3}
\end{figure*}



% \begin{figure*}[t]
% 	% \begin{subfigure}[b]{0.48\linewidth}%
%         \centering
%     % \begin{subfigure}[t]{0.5\columnwidth}%h
%     % 	\center
%     %     \captionsetup{justification=centering}
%     %     % \includegraphics[width=\linewidth]{figures/plots/experiment/ev-1-usertxn-latency.pdf}        
%     %     \includegraphics[width=\linewidth]{figures/plots/motivation/2_moti_nothing_zk.png}        
%     %  \caption{Segragated Storage on Shared-Nothing}
%     %     \label{fig:lw_migr_user_throughput}
%     % \end{subfigure}%
%     \begin{subfigure}[b]{0.5\linewidth}%
%     	\center
%         \captionsetup{justification=centering}
%         % \includegraphics[width=\linewidth]{figures/plots/experiment/ev-1-usertxn-latency.pdf}        
%         \includegraphics[width=\columnwidth]{figures/plots/2_moti/2_moti_f1_a.pdf}        

%      \caption{Segragated Storage on Shared-Nothing}
%         \label{fig:moti_f1_a}
%     \end{subfigure}%
%     % \vspace{.3in}
%     % \begin{subfigure}[t]{0.8\columnwidth}%
%     % 	\center
%     %     \captionsetup{justification=centering}
%     %     \includegraphics[width=\linewidth]{figures/plots/2_moti/2_moti_f1_b.pdf}        

%     %  \caption{Segragated Storage on Storage Disaggregation}
%     %     \label{fig:moti_f1_b}
%     % \end{subfigure}%
%     % \vspace{.3in}
%     \begin{subfigure}[b]{0.5\linewidth}%
%     	\center
%         \captionsetup{justification=centering}
%         \includegraphics[width=\columnwidth]{figures/plots/2_moti/2_moti_f1_c.pdf}        

%      \caption{Unified Storage on Storage Disaggregation}
%         \label{fig:moti_f1_c}
%     \end{subfigure}%
%     % \vspace{-.15in}
%     % \setlength{\belowcaptionskip}{-10pt}
%     % \setlength{\abovecaptionskip}{-10pt}

%     \caption{\textbf{DBMS Architectures for Cluster Management} --- \normalfont{The green boxes are the auxiliary services. The control plane is not shown for simplicity.}
%     \yxy{a few extra suggestions: (1) the nodes can be narrower (if need space). (2) the green part in Figure 1(a) can look a little different from the other parts; right now it looks a bit like the system state is a third partition of the cluster.}
%     }
%     \label{fig:moti_f1}
% \end{figure*}




==> figures/plots_code/2_motivation/migration-compr.tex <==
% \begin{table*}[th]
%     \begin{center}
%     \caption{Performance Degradation Analysis}
%     \label{tbl:moti_migr_cmpr}
%     \vspace{-3mm}
%     \small
%     \begin{tabular}{ l l l l l l l l l }
%     \toprule
%     \multicolumn{1}{c}{} &\multicolumn{5}{c}{\textbf{Push Reconfiguration}} && \multicolumn{2}{c}{\textbf{Pull Reconfiguration}} \\
%     \cline{2-6}   \cline{8-9}  
%     \textbf{Indicators} & \textcolor{red}{\textbf{\system(Hybrid-Heat)}} & \textbf{Lock \& Abort} & \textcolor{red}{\textbf{Albatross}} & \textbf{DynaMast} & \textbf{Remus} && \textbf{\system (Post-Heat)} & \textbf{Squall} \\ 
%     \midrule
%     Transaction Abort & Partial & All & No & No & No && No & All\\
%     Service Downtime & Short & Long & Long & Long & No && Short & No\\
%     % Service Downtime & Yes & Yes & Yes & Yes & No && Yes & No\\
%     Cache Miss & No & No & No & No & No && Yes & Yes\\
%     Isolation Level & S & S & S & SI & SI && S & S\\

%     \bottomrule
%     \end{tabular}
%     \end{center}
%     \end{table*}


\begin{table}[th]
    \begin{center}
    \centering
    % \caption{Performance Degradation Analysis}
     \setlength{\tabcolsep}{2pt}
    % \vspace{-3mm}
    \small
    \begin{tabular}{ l l l l l l }
    \toprule
    % \multicolumn{1}{c}{} &\multicolumn{5}{c}{\textbf{PreHeat}} && \multicolumn{1}{c}{\textbf{PostHeat}} \\
    % \cline{2-6}   \cline{8-8}  
    % \textbf{Indicators} & \textbf{\system} & \textbf{Albatross} & \textbf{DynaMast} & \textbf{Remus} && \textbf{Squall} \\ 
    % \midrule
    % Transaction Abort & All & No & No & No && All\\
    % Service Downtime  & Minimal & Yes & Yes & No && No\\
    % Cache Miss No & No & No & No && Yes\\
    % Isolation Level  S & S & SI & SI && S\\

    \textbf{Indicators}&\textbf{\system}&\textbf{DynaMast}&\textbf{Albatross}&\textbf{Squall}&\textbf{Remus} \\ 
    \midrule
    \# of CC protocols & 1 & 2 & 2 & 2 & 2\\
    Transaction Abort & Yes & No & No & Yes & No\\
    Service Downtime  & Minimal & Yes & Yes & Minimal & No\\
    $N_{dst}$ Cache Miss &No & No & No & Yes & No\\
    Isolation Level  &S & SI & S & S & SI\\


    \bottomrule
    \end{tabular}
    \vspace{3mm}
    % \setlength{\belowcaptionskip}{-10pt}
    \setlength{\abovecaptionskip}{-10pt}
    \caption{Reconfiguration Costs Analysis}
    \end{center}
    \label{tbl:moti_t1}
\end{table}

==> figures/plots_code/3_architecture/f2.tex <==
\begin{figure}[h!]
    \begin{subfigure}{0.5\columnwidth}%
        \centering
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/3_architecture/3_overview_f2_a.pdf}  
        \caption{Unpartitioned Metadata}
        \label{fig:arch_f2_a}
    \end{subfigure}%
    % \par\medskip
    % \hfill
    \begin{subfigure}{0.5\columnwidth}%
        \centering
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/3_architecture/3_overview_f2_b.pdf}  
        \caption{Unowned Metadata Parititon}
        \label{fig:arch_f2_b}
    \end{subfigure}%

    \vspace{-.10in}
    \setlength{\belowcaptionskip}{-5pt}
    \caption{Inconsistency Risks.}

    \label{fig:arch_f2}
    % \vspace{-.1 in}
\end{figure}

==> figures/plots_code/4_cluster_management/c1_interface.tex <==
\begin{algorithm}[t!]
	\small 
    \SetKwProg{myfun}{Function}{}{}
    \SetKwProg{begintxn}{BEGIN TXN}{}{}
    \SetKwProg{committxn}{COMMIT TXN}{}{}
    \SetKwProg{aborttxn}{ON ERROR}{}{}


    \nonl\texttt{\\}
    \myfun{\textbf{Append(target\_lsn)}}{  
       \While{true} {
         \textit{(new\_lsn, delta)  $\leftarrow$ Syslog.ReadToTail(cur\_lsn)} \\  
         \uIf{delta not empty}{
           \textit{MTable.MembershipCatchUp(delta) } \\
           \textit{cur\_lsn $\leftarrow$ new\_lsn} \\
         }
        \textit{Sleep(polling\_interval) } \\
      }   
    }

    \nonl\texttt{\\}
    \myfun{\textbf{DeleteNode()}}{  
       \While{true} {
         \textit{(new\_lsn, delta)  $\leftarrow$ ReadToTail(cur\_lsn)} \\  
         \uIf{delta not empty}{
           \textit{MembershipCatchUp(delta) } \\
           \textit{cur\_lsn $\leftarrow$ new\_lsn} \\
         }
        \textit{Sleep(polling\_interval) } \\
      }   
    }

    \nonl\texttt{\\}



    \myfun{\textbf{MemberSynchronization()}}{  
    \While{true} {
      \textit{(new\_lsn, delta)  $\leftarrow$ Syslog.ReadToTail(cur\_lsn)} \\  
      \uIf{delta not empty}{
        \textit{MTable.MembershipCatchUp(delta) } \\
        \textit{cur\_lsn $\leftarrow$ new\_lsn} \\
      }
     \textit{Sleep(polling\_interval) } \\
    }   
    }
    % \nonl\texttt{\\}


    \myfun{\textbf{HealthMonitorThread(node\_addr)}}{     
      \While{true} {
        \textit{(new\_lsn, delta)  $\leftarrow$ ReadToTail(cur\_lsn)} \\  
        \uIf{delta not empty}{
          \textit{MembershipCatchUp(delta) } \\
          \textit{cur\_lsn $\leftarrow$ new\_lsn} \\
        }
       \textit{Sleep(polling\_interval) } \\
      }  
    }

    % \nonl\texttt{\\}





    % \myfun{\textbf{PerformanceMonitor(node\_addr)}}{     
    %   \textit{new\_node\_id  $\leftarrow$ MTable.getMaxNodeID() + 1} \\  
    %   \For{nid in MTable} {
    %     \textit{{RPC$_{\textit{nid}}$::MTable.insert(new\_node\_id, node\_addr)}}\\
    %     % \textit{MTable.insert(nid, Addr3) } \
    %   }
    %       % \nonl \codeComment{has\_system\_participant is true} \\
    %     \textit{Marlin2PC.commit() } \\
    %   }
    %   \nonl\texttt{\\}


 
    \caption{\textbf{Membership Management Protocol using \name}}
     
    % \caption{\textbf{MigrationTxn in \name} --- Nodes is a list containing two node participants. When there is no node failure, nodes contain the node\_src the node\_dst. When node\_src has failed, nodes contain the node\_disc(the node discovered the failure) the node\_dst. g is the granule to be migrated }

    \label{alg:cluster_c1}

\end{algorithm}

==> figures/plots_code/4_cluster_management/c1_membership.tex <==
\begin{algorithm}[t!]
	\small 
    \SetKwProg{myfun}{Function}{}{}

    \nonl\texttt{\\}
    
    % \myfun{\textbf{HealthMonitor()}}{     
    %   \While{true} {
    %     % \textit{response $\leftarrow$ SendHeartBeatTo(node)} \\
    %     \textit{response $\leftarrow$ TryLog(cur\_glog, HEART\_BEAT)} \\
    %     \uIf{response is \texttt{Abort} and not MTable.exist(cur\_node)} {
    %         \textit{terminate cur\_node} \\
    %     }
    %     \Else {
    %       \textit{Sleep(heartbeat\_interval) } \\
    %     }
    %   }  
    % }

    \myfun{\textbf{HealthMonitor(node)}}{     
      \While{true} {
        % \textit{response $\leftarrow$ SendHeartBeatTo(node)} \\
        \textit{response $\leftarrow$ RPC$_{\textit{sync}}^{\textit{node}}$::SendHeartbeat()} \\
        \uIf{response is \texttt{Timeout}} {
            \uIf{consecutive\_timeout $>$ threshold} {
              \textit{Failover(node, cur\_node)} \\
              \textit{consecutive\_timeout $\leftarrow$ 0} \\
            }
            \Else{
              \textit{consecutive\_timeout+=heartbeat\_interval} \\
            }
        }
        \ElseIf{response is \texttt{ACK}} {
          \textit{Sleep(heartbeat\_interval) } \\
        }
      }  
    }

    \myfun{\textbf{Failover(failed\_node, recovery\_node)}}{     
       \textit{DeleteNodeTxn(failed\_node)} \\
       \nonl \codeComment{Broadcast is optional} \\
       \textit{RPC$_{\textit{async}}^{\textit{cluster}}$::Broadcast(DELETE\_NODE)} \\
       \textit{RecoveryMigrTxn(granules, failed\_node, recovery\_node)} \\
       \textit{RPC$_{\textit{async}}^{\textit{cluster}}$::Broadcast(MIGR\_GRANULE)} \\
    }
    \nonl\texttt{\\}

    \myfun{\textbf{MemberSync()}}{  
    \While{true} {          
      \textit{MetaRefresh(Syslog)} \\
      \textit{Sleep(refresh\_interval) } \\
    }   
    }

    % \nonl\texttt{\\} 
    \caption{\textbf{Membership Management in \system}}

    \label{alg:groupmem_c1}

\end{algorithm}

==> figures/plots_code/4_cluster_management/c2.tex <==
\begin{algorithm}[t!]
	\small 
    \SetKwProg{myfun}{Function}{}{}
    \nonl\texttt{\\}      
    \myfun{Coordinator::Start2PC(participants, \hl{has\_sys\_participant})}{ 
           	\For{p in participants} {
    		\textbf{send} \texttt{VOTE-REQ} to $p$ asynchronously \\
    	}

      \If{ \hl{ has\_sys\_participant}} {
         \nonl \codeComment{log vote on \syslog} \\

          \hl{\textit{sys\_vote $\leftarrow$ 
 Logger::LogVote(\syslog, \texttt{VOTE-YES})}}\\
          }
     
         \textbf{wait for }\textit{all votes from \hl{participants and sys\_participant}} \\
    	\Indp 
    	      \textbf{on receiving \texttt{ABORT}} \textit{decision $\leftarrow$ \texttt{ABORT}} \\              
    	      \textbf{on receiving all responses} \textit{decision $\leftarrow$ \texttt{COMMIT}} \\
              \textbf{on timeout } \textit{decision $\leftarrow$ TerminationProtocol(txn)} \\
        \Indm
    	\textit{reply decision to the txn caller} \\
        %\textit{RPC$_{\textit{\hl{async}}}^{\textit{local log}}$::Log(decision)} \\
    	\For{p in txn.participants}{
            \textbf{send} \textit{decision} to p asynchronously \\
    	}
            	\textit{RPC$_{\textit{sync}}^{\textit{ sys log}}$::Append(decision)}
    }

    \nonl\texttt{\\}
      \caption{\textbf{Marlin2PC} --- Differences between Marlin2PC and standard 2PC are highlighted in \hl{gray}.}
    \label{alg:cluster_c2}

\end{algorithm}


==> figures/plots_code/4_cluster_management/f1_old.tex <==


\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/plots/4_clustermanagement/f1.pdf}
    \setlength{\abovecaptionskip}{-5pt}
    \setlength{\belowcaptionskip}{-5pt}
 
    \caption{System Tables (MTable and GTable) --- \normalfont{This figure only shows system states. Arrows denote access flow.}}
    \label{fig:systbl_f1}
    % \vspace{-.1 in}
\end{figure}

==> figures/plots_code/4_cluster_management/f2.tex <==
% \begin{figure}[h!]
%     \begin{subfigure}[t]{0.48\columnwidth}%
%         \centering
%         % \captionsetup{justification=centering}
        
%         \includegraphics[width=\linewidth]{figures/plots/4_clustermanagement/f2_a.png}
%         \caption{Normal Case}
%         \label{fig:arch_f2_a}
%     \end{subfigure}%
%         \hfill

%     \begin{subfigure}[t]{0.48\columnwidth}%
%         \centering
%         % \captionsetup{justification=centering}
%         \includegraphics[width=\linewidth]{figures/plots/4_clustermanagement/f2_b.png}
%         \caption{Failure Case}
%         \label{fig:arch_f2_b}
%     \end{subfigure}%

%         % \hfill
%     % \hspace{.10in}


%     % \vspace{-.10in}
%     \setlength{\belowcaptionskip}{-5pt}
%     \caption{Granule Ownership Table (GTable) --- \normalfont{This figure only shows coordination states. Arrows denote access flow.}}

%     \label{fig:arch_f2}
%     % \vspace{-.1 in}
% \end{figure}


\begin{figure}[h!]
    \begin{subfigure}{0.5\columnwidth}%
        \centering
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/4_clustermanagement/f2_a.png}
        \caption{Normal Case}
        \label{fig:arch_f2_a}
    \end{subfigure}%
    % \par\medskip
    \hfill
    \begin{subfigure}{0.5\columnwidth}%
        \centering
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/4_clustermanagement/f2_b.png} 
        % \caption{Unowned Metadata Parititon}
        \caption{Failure Case}
        \label{fig:arch_f2_b}
    \end{subfigure}%

    \vspace{-.10in}
    \setlength{\belowcaptionskip}{-5pt}
    \caption{Granule Ownership Table (GTable) --- \normalfont{This figure only shows coordination states. Arrows denote access flow.}}


    \label{fig:systbl_f2}
    % \vspace{-.1 in}
\end{figure}

==> figures/plots_code/4_cluster_management/f2_old.tex <==

\begin{figure}[h]
	% \begin{subfigure}[b]{0.48\linewidth}%
        \centering

    \begin{subfigure}[t]{0.9\columnwidth}%
    	\center
        % \captionsetup{justification=centering}
        % \includegraphics[width=\linewidth]{\hybirdtl-1.pdf}  
        % \includegraphics[width=\linewidth]{\hybirdtl-2.pdf}  
        % \includegraphics[width=\linewidth]{\hybirdtl-4.pdf}  
        % \includegraphics[width=\linewidth]{\hybirdtl-8.pdf}  
        \includegraphics[width=\linewidth]{figures/plots/4_clustermanagement/f2_a.pdf}
        % \includegraphics[width=\linewidth]{\hybirdtl-32.pdf}  
        \caption{AddNodeTxn}
        \label{fig:cluster_f2_a}
    \end{subfigure}%
    \par\medskip
    \begin{subfigure}[t]{0.9\columnwidth}%
    	\center
        % \captionsetup{justification=centering}
        % \includegraphics[width=\linewidth]{\preheattl-1.pdf}  
        % \includegraphics[width=\linewidth]{\preheattl-2.pdf}  
        % \includegraphics[width=\linewidth]{\preheattl-4.pdf}  
        % \includegraphics[width=\linewidth]{\preheattl-8.pdf}  
        \includegraphics[width=\linewidth]{figures/plots/4_clustermanagement/f2_b.pdf}
        % \includegraphics[width=\linewidth]{\preheattl-32.pdf}
     \caption{MigrationTxn}
     \label{fig:cluster_f2_b}
    \end{subfigure}%
    % \vspace{-.15in}
    % \setlength{\belowcaptionskip}{-10pt}
    \caption{Illustration of Reconfiguration Transactions}
    \label{fig:cluster_f2}
\end{figure}


==> figures/plots_code/4_cluster_management/f3_examples_failover.tex <==
\begin{figure}[h]
        \vspace{-.10in}

    \centering
    % \includegraphics[width=0.8\linewidth]{figures/plots/4_clustermanagement/f1.png}
    \includegraphics[width=0.7\linewidth]{figures/plots/4_examples/4_example_failover1.png}
    % \setlength{\abovecaptionskip}{-5pt}
    % \setlength{\belowcaptionskip}{-10pt}
    \vspace{-.1 in}
    % \setlength{\abovecaptionskip}{-.05in}
    \caption{Failover Example}
    \vspace{-.1 in}

    \label{fig:failover}
    % \vspace{-.1 in}
\end{figure}

==> figures/plots_code/4_cluster_management/x.tex <==


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/plots/4_clustermanagement/newprotocol.pdf}
    \setlength{\abovecaptionskip}{-5pt}
    \setlength{\belowcaptionskip}{-5pt}
 
    % \caption{System Tables (MTables and GTables) --- \normalfont{Cells in red are granules located on the owner compute node.}}
    \label{fig:cluster_x}
    % \vspace{-.1 in}
\end{figure}

==> figures/plots_code/5_faulttolerance/f1.tex <==

\begin{figure}[h]
	% \begin{subfigure}[b]{0.48\linewidth}%
        \centering

        \includegraphics[width=0.9\linewidth]{figures/plots/5_faulttolerance/f1.pdf}

    % \vspace{-.15in}
    % \setlength{\belowcaptionskip}{-10pt}
    \caption{Illustration of Node Failure --- \normalfont{Red blocks are updates of \textit{DeleteNodeTxn}
    % \yxy{in step \textcircled{4}, p1 should be P1.}
    }}
    \label{fig:ft_f1}
\end{figure}


==> figures/plots_code/5_optimization/c1.tex <==
\begin{algorithm}[t!]
	\small 
    \SetKwProg{myfun}{Function}{}{}
    \nonl\texttt{\\}

    \myfun{\textbf{MigrationTxn(G1, N1, N3)}}{ 
      \hl{\textit{{RPC$_{\textit{N1}}$::Copy(G1)}}}\\
    %   \hl{\textit{Cache.heat(G1)}} \\
       \nonl \codeComment{ownership transfer start} \\
        \textit{node $\leftarrow$ GTable.get(G1, "NodeID")} \\
        \If{node is N1} {
             \nonl \codeComment{implicitly acquire an exclusive lock for G1 on GTable} \\
             \textit{GTable.update(G1, "NodeID", N3)}\\
        }
        \textit{Marlin2PC.commit(true) } \\
        \nonl \codeComment{ownership transfer finished} \\
        \hl{\textbf{wait for} \textit{\texttt{final\_updates\_keys}} \textbf{from} \textit{N1}}\\
        \hl{\textit{LockTable.acquire(UserTable, keys)}}\\
        \hl{\textit{LockTable.release(GTable, G1)}}\\
        \nonl \codeComment{final updates synchronization} \\
        \hl{\textbf{wait for} \textit{final\_updates} \textbf{from} \textit{N1}}\\
        \hl{\textit{LockTable.release(UserTable, keys)}}\\ 
    }
    \nonl\texttt{\\}

 
    \caption{\textbf{Optimized MigrationTxn} --- Differences between optimized \textit{MigrationTxn} and naive \textit{MigrationTxn} are highlighted in \hl{gray}.}
     
    % \caption{\textbf{MigrationTxn in \name} --- Nodes is a list containing two node participants. When there is no node failure, nodes contain the node\_src the node\_dst. When node\_src has failed, nodes contain the node\_disc(the node discovered the failure) the node\_dst. g is the granule to be migrated }

    \label{alg:optimization_c1}

\end{algorithm}

==> figures/plots_code/5_optimization/c2.tex <==
\begin{algorithm}[t!]
	\small 
    \SetKwProg{myfun}{Function}{}{}
    \nonl\texttt{\\}

    \myfun{\textbf{MigrationTxn(G1, N1, N3)}}{ 
       \nonl \codeComment{ownership transfer start} \\
        \textit{node $\leftarrow$ GTable.get(G1, "NodeID")} \\
        \If{node is N1} {
             \textit{GTable.update(G1, "NodeID", N3)}\\
        }
        \textit{Marlin2PC.commit(true) } \\
        \nonl \codeComment{ownership transfer finished} \\
        \nonl \codeComment{heat the cache on destination node} \\
        \hl{\textit{UserTable.scan(G1)}}\\
    }
    \nonl\texttt{\\}

 
    \caption{\textbf{MigrationTxn(Postheat)} --- \wjh{separate it into two transactions?}Differences between optimized \textit{MigrationTxn} and naive \textit{MigrationTxn} are highlighted in \hl{gray}.}
     
    % \caption{\textbf{MigrationTxn in \name} --- Nodes is a list containing two node participants. When there is no node failure, nodes contain the node\_src the node\_dst. When node\_src has failed, nodes contain the node\_disc(the node discovered the failure) the node\_dst. g is the granule to be migrated }

    \label{alg:optimization_c2}

\end{algorithm}

==> figures/plots_code/5_optimization/f1.tex <==
\begin{figure}[h]
	% \begin{subfigure}[b]{0.48\linewidth}%
        \centering

        \includegraphics[width=0.8\linewidth]{figures/plots/5_optimization/f1.pdf}

    \vspace{-.15in}
    \setlength{\belowcaptionskip}{-12pt}
    \caption{Unavailability Window in Migration}
    % \caption{Unavailability Window in Migration \yxy{(1) Call left figure "Coarse-Grained Sync" instead of "Cache Preheat"? (2) Also, mark the orange part as granule lock? (3) this figure is taking a lot of space. Try to shrink it. BTW, try to keep the fontsize in figures similar to the front size in text. Right now the text in Figure 6 is a little big.}
    % }
    \label{fig:optimization_f1}
\end{figure}


==> figures/plots_code/5_recipe/c1_migr.tex <==
\begin{algorithm}[t!]
	\small 
    \SetKwProg{myfun}{Function}{}{}

    \nonl\texttt{\\}
    \nonl \codeComment{Assume the transaction is triggered on the destination node} \\
    \myfun{\textbf{MigrationTxn(granule, src, dst)}}{ 
      \textit{{nid $\leftarrow$ RPC$_{\textit{src}}$::GTable[granule].NodeID}}\\ 
      \uIf{nid is src} {
        \textit{{RPC$_{\textit{async}}^{\textit{src}}$::GTable[granule].NodeID = dst}}\\ 
        \textit{GTable[granule].NodeID = dst}\\
        \textit{reply to caller \textit{\mcommit(\{src, dst\}) }} \\
        \hl{\textit{granule\_data $\leftarrow$ RPC$_{\textit{async}}^{\textit{src}}$::UserTableCache.scan(granule)}} \\
        \hl{\textit{UserTableCache.insert(granule\_data)}} \\
      }
      \Else{\textit{\textbf{Abort} and \Return WrongNodeError(nid)} }
    }
    % \nonl \codeComment{Assume the transaction is triggered on the source node} \\
    % \myfun{\textbf{MigrationTxn(granule, src, dst)}}{ 
    %   \textit{nid  $\leftarrow$ GTable[granule].NodeID}\\
    %   \uIf{nid is src} {
    %     % \textit{lsn $\leftarrow$ Log.getLSN()} \\
    %     \textit{{RPC$_{\textit{dst}}$::GTable[granule].NodeID = dst}}\\ 
    %     \textit{GTable[granule].NodeID = dst}\\
    %     % \textit{Log.replayCatchUp(lsn)} \\
    %     \Return \textit{\mcommit(\{src, dst\}) } \\
    %   }
    %   \Else{\textit{\textbf{Abort} and \Return WrongNodeError(nid)} }
    % }
    
    % \nonl\texttt{\\}
    % \nonl \codeComment{The transaction is triggered on the destination node} \\
    % \myfun{\textbf{RecoveryMigrTxn(granule, src, dst)}}{ 
    %    \textit{GTable[granule].NodeID = dst}\\
    %    \textit{\mcommit(\{src.Glog, dst\}) } \\
    % }
    
    \caption{\textbf{Live Migration using \system}}
    % \caption{\textbf{Transactional Reconfigurations using \textit{MarlinCommit}} --- Differences between \system UserTxn and standard UserTxn are highlighted in \hl{gray}.}
     

    \label{alg:livemigration_c1}

\end{algorithm}

==> figures/plots_code/experiments/EV1/f1_old.tex <==
\begin{figure}
	% \begin{subfigure}[b]{0.48\linewidth}%
    % \newcommand{\patha}{figures/plots/experiment/rampup}
    % \begin{subfigure}[b]{0.9\linewidth}%
    	% \center
        % \captionsetup{justification=centering}
        % \includegraphics[width=0.9\linewidth]{figures/plots/experiment/ev3-scaleup.pdf}
        % % \caption{Throughput Overtime}
        % \label{fig:ev1_f1_a}
    	\begin{subfigure}{0.9\columnwidth}%
            \centering
            % \captionsetup{justification=centering}
            \includegraphics[width=\linewidth]{figures/plots/experiment/ev1-tradeoff.pdf}  
            \caption{Cost per Transaction vs. Migration Duration}
            \label{fig:ev1_f1_a}
        \end{subfigure}%
        % \par\medskip
        \hfill
        \begin{subfigure}{0.9\columnwidth}%
            \centering
            % \captionsetup{justification=centering}
            \includegraphics[width=\linewidth]{figures/plots/experiment/ev1-tradeoff-throughput.pdf}  
            \caption{Cost per Transaction vs. Migration Throughput}
            \label{fig:ev1_f1_b}
        \end{subfigure}%

    \vspace{-.10in}
    \setlength{\belowcaptionskip}{-5pt}
    \caption{Cost vs. Migration Performance Tradeoff.}
    % \caption{Performance on Scale-Out Workload of \system Versus On-premise Clusters}
    \label{fig:ev1_f1}
\end{figure}





==> figures/plots_code/experiments/EV1/f2_old.tex <==
\begin{figure}
    % \centering
	\begin{subfigure}{0.5\columnwidth}%
    	\centering
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev1-cost-breakdown.png}  
        \caption{Cost Breakdown}
        \label{fig:ev1_f2_a}
    \end{subfigure}%
    % \par\medskip
    \hfill
    \begin{subfigure}{0.5\columnwidth}%
    	\centering
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev1-migr-latency-breakdown.png}  
        \caption{Migration Transaction Latency Breakdown}
        \label{fig:ev1_f2_b}
    \end{subfigure}%
    % \vspace{-.15in}
    % \setlength{\belowcaptionskip}{-10pt}
    \caption{Performance Breakdown}
    \label{fig:ev1_f2}
\end{figure}

==> figures/plots_code/experiments/EV1/f3_old.tex <==



\begin{figure}[h]
	% \begin{subfigure}[b]{0.48\linewidth}%
        \centering
    \newcommand{\usrmarlin}{figures/plots/experiment/ev1-usr-timeline-Marlin.pdf}
    \newcommand{\migrmarlin}{figures/plots/experiment/ev1-migr-timeline-Marlin.pdf}
    \newcommand{\usrszk}{figures/plots/experiment/ev1-usr-timeline-Small-ZK.pdf}
    \newcommand{\migrszk}{figures/plots/experiment/ev1-migr-timeline-Small-ZK.pdf}
    \newcommand{\usrlzk}{figures/plots/experiment/ev1-usr-timeline-Large-ZK.pdf}
    \newcommand{\migrlzk}{figures/plots/experiment/ev1-migr-timeline-Large-ZK.pdf}

    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        \includegraphics[width=\linewidth]{\usrmarlin}  
        \caption{User Txn Throughtput for \system}

        \label{fig:ev1-f3-a}
    \end{subfigure}%
    % \par\medskip
    % \begin{subfigure}[t]{0.95\columnwidth}%
    % 	\center
    %     \includegraphics[width=\linewidth]{\migrmarlin}  
    %  \caption{Migration Throughtput for \system}

    %  \label{fig:ev1-f3-b}
    % \end{subfigure}%
    \par\medskip
    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        \includegraphics[width=\linewidth]{\usrszk}  
        \caption{User Txn Throughtput for Small Zookeeper}
     \label{fig:ev1-f3-c}
    \end{subfigure}%
    \par\medskip
    % \begin{subfigure}[t]{0.95\columnwidth}%
    % 	\center
    %     \includegraphics[width=\linewidth]{\migrszk}  
    %  \caption{Migration Throughput for Small Zookeeper}    
    %   \label{fig:ev1-f3-d}
    % \end{subfigure}%
    % \par\medskip
    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        \includegraphics[width=\linewidth]{\usrlzk}  
     \caption{User Txn Throughtput for Large Zookeeper}
     \label{fig:ev1-f3-e}
    \end{subfigure}%
    % \par\medskip
    % \begin{subfigure}[t]{0.95\columnwidth}%
    % 	\center
    %     \includegraphics[width=\linewidth]{\migrlzk}  
    %  \caption{Migration Throughput for Large Zookeeper}
    %  \label{fig:ev1-f3-f}
    % \end{subfigure}%
    % \vspace{-.15in}
    % \setlength{\belowcaptionskip}{-10pt}
      \par\medskip
    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev1-realtime-migr.png}  
     \caption{Migration Transaction Throughput}
     \label{fig:ev1-f3-f}
    \end{subfigure}%
    \caption{Throughput Over Time During Reconfiguration}
    \label{fig:ev1-f3}
\end{figure}


==> figures/plots_code/experiments/EV2/f1_old.tex <==



\begin{figure}[h]
	% \begin{subfigure}[b]{0.48\linewidth}%
        \centering
    \newcommand{\usrmarlin}{figures/plots/experiment/ev3-dynamic-throughput.png}
    \newcommand{\migrmarlin}{figures/plots/experiment/ev3-dynamic-latency.png}
    \newcommand{\usrszk}{figures/plots/experiment/ev3-dynamic-abort.png}
    \newcommand{\migrszk}{figures/plots/experiment/ev3-dynamic-migr-tps.png}
    \newcommand{\usrlzk}{figures/plots/experiment/ev3-dynamic-realtime-cost.png}
    % \newcommand{\migrlzk}{figures/plots/experiment/ev3-migr-timeline-Large-ZK.pdf}

    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        \includegraphics[width=\linewidth]{\usrmarlin}  
        \caption{User Txn Throughtput}

        \label{fig:ev2-f1-a}
    \end{subfigure}%
    \par\medskip
    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        \includegraphics[width=\linewidth]{\migrmarlin}  
     \caption{User Txn Latency}

     \label{fig:ev2-f1-b}
    \end{subfigure}%
    \par\medskip
    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        \includegraphics[width=\linewidth]{\usrszk}  
        \caption{User Txn Abort Rate}
     \label{fig:ev2-f1-c}
    \end{subfigure}%
    \par\medskip
    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        \includegraphics[width=\linewidth]{\migrszk}  
     \caption{Migration Txn Throughput}    
      \label{fig:ev2-f1-d}
    \end{subfigure}%
    \par\medskip
    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        \includegraphics[width=\linewidth]{\usrlzk}  
     \caption{Realtime Cost}
     \label{fig:ev2-f1-e}
    \end{subfigure}%
    % \vspace{-.15in}
    % \setlength{\belowcaptionskip}{-10pt}
    \caption{Realtime Performance During Dynamic Workloads}
    \label{fig:ev2-f1}
\end{figure}


==> figures/plots_code/experiments/EV2/f2_old.tex <==
\begin{figure}
    % \centering
	% \begin{subfigure}{0.\columnwidth}%
    	\centering
        % \captionsetup{justification=centering}
        \includegraphics[width=0.8\linewidth]{figures/plots/experiment/ev3-dynamic-cost-dur-bar.png}  
    %     \captioVn{Cost Breakdown}
    %     \label{fig:ev2_f2_a}
    % \end{subfigure}%
    % \par\medskip
    % \hfill
    % \begin{subfigure}{0.5\columnwidth}%
    % 	\centering
    %     % \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{figures/plots/experiment/ev1-migr-latency-breakdown.png}  
    %     \caption{Migration Transaction Latency Breakdown}
    %     \label{fig:ev2_f2_b}
    % \end{subfigure}%
    % \vspace{-.15in}
    % \setlength{\belowcaptionskip}{-10pt}
    \caption{Comparison of Cost and Migration Duration}
    \label{fig:ev2_f2}
\end{figure}

==> figures/plots_code/experiments/EV4/f2.tex <==
\begin{figure}
    % \centering
	% \begin{subfigure}{0.\columnwidth}%
    	\centering
        % \captionsetup{justification=centering}
        \includegraphics[width=0.8\linewidth]{figures/plots/experiment/ev4-dynamic-cost-dur-bar.png}  
    %     \captioVn{Cost Breakdown}
    %     \label{fig:ev2_f2_a}
    % \end{subfigure}%
    % \par\medskip
    % \hfill
    % \begin{subfigure}{0.5\columnwidth}%
    % 	\centering
    %     % \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{figures/plots/experiment/ev1-migr-latency-breakdown.png}  
    %     \caption{Migration Transaction Latency Breakdown}
    %     \label{fig:ev2_f2_b}
    % \end{subfigure}%
    % \vspace{-.15in}
    % \setlength{\belowcaptionskip}{-10pt}
    \caption{Comparison of Cost and Migration Duration}
    \label{fig:ev4_f2}
\end{figure}

==> figures/plots_code/experiments/EV5/f1_old_failover.tex <==
\begin{figure}[h]
	% \begin{subfigure}[b]{0.48\linewidth}%
    \centering
    % \begin{subfigure}[t]{0.95\columnwidth}%
    	% \center
        % \includegraphics[width=\linewidth]{figures/plots/experiment/ev5-failover-througput.png}  
    %  \caption{Migration Transaction Throughput}
    %  \label{fig:ev5-f1-a}
    % \end{subfigure}%
    \begin{subfigure}[t]{\columnwidth}%
    	\center
        \includegraphics[width=0.95\linewidth]{figures/plots/experiment/ev5-failover32-througput.png}  
        \caption{User Txn Throughtput}

        \label{fig:ev5-f1-a}
    \end{subfigure}%
    \par\medskip
    \begin{subfigure}[t]{\columnwidth}%
    	\center
        \includegraphics[width=0.95\linewidth]{figures/plots/experiment/ev5-failover32-migr-throughput.png}  
     \caption{Migration Txn Throughput}

     \label{fig:ev5-f1-b}
    \end{subfigure}%
    \setlength{\belowcaptionskip}{-10pt}
    \caption{Throughput under Failover}
    \label{fig:ev5-f1}
\end{figure}

==> figures/plots_code/experiments/Obsolete/EV1/f1.tex <==



\begin{figure}[h]
	% \begin{subfigure}[b]{0.48\linewidth}%
        \centering
    \newcommand{\marlintl}{figures/plots/experiment/ev1-throughput-timeline-marlin.pdf}
    \newcommand{\dynamasttl}{figures/plots/experiment/ev1-throughput-timeline-dynamast.pdf}
    \newcommand{\albatrosstl}{figures/plots/experiment/ev1-throughput-timeline-albatross.pdf}
    \newcommand{\postheattl}{figures/plots/experiment/ev1-throughput-timeline-postheat.pdf}

    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        % \captionsetup{justification=centering}
        % \includegraphics[width=\linewidth]{\hybirdtl-1.pdf}  
        % \includegraphics[width=\linewidth]{\hybirdtl-2.pdf}  
        % \includegraphics[width=\linewidth]{\hybirdtl-4.pdf}  
        % \includegraphics[width=\linewidth]{\hybirdtl-8.pdf}  
        \includegraphics[width=\linewidth]{\marlintl}  
        % \includegraphics[width=\linewidth]{\hybirdtl-32.pdf}  
        \caption{\system}
        \label{fig:ev1-f1-a}
    \end{subfigure}%
    \par\medskip
    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        % \captionsetup{justification=centering}
        % \includegraphics[width=\linewidth]{\preheattl-1.pdf}  
        % \includegraphics[width=\linewidth]{\preheattl-2.pdf}  
        % \includegraphics[width=\linewidth]{\preheattl-4.pdf}  
        % \includegraphics[width=\linewidth]{\preheattl-8.pdf}  
        \includegraphics[width=\linewidth]{\dynamasttl}  
        % \includegraphics[width=\linewidth]{\preheattl-32.pdf}
     \caption{DynaMast}
     \label{fig:ev1-f1-b}
    \end{subfigure}%
    \par\medskip
    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        % \captionsetup{justification=centering}
        % \includegraphics[width=\linewidth]{\postheattl-1.pdf}  
        % \includegraphics[width=\linewidth]{\postheattl-2.pdf}  
        % \includegraphics[width=\linewidth]{\postheattl-4.pdf}  
        % \includegraphics[width=\linewidth]{\postheattl-8.pdf}  
        \includegraphics[width=\linewidth]{\albatrosstl}  
        % \includegraphics[width=\linewidth]{\postheattl-32.pdf}
     \caption{Albatross}
     \label{fig:ev1-f1-c}
    \end{subfigure}%
    \par\medskip
    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        % \captionsetup{justification=centering}
        % \includegraphics[width=\linewidth]{\noheattl-1.pdf}  
        % \includegraphics[width=\linewidth]{\noheattl-2.pdf}  
        % \includegraphics[width=\linewidth]{\noheattl-4.pdf}  
        % \includegraphics[width=\linewidth]{\noheattl-8.pdf}  
        \includegraphics[width=\linewidth]{\postheattl}  
        % \includegraphics[width=\linewidth]{\noheattl-32.pdf}
     \caption{Squall}
     \label{fig:ev1-f1-d}
    \end{subfigure}%
    % \vspace{-.15in}
    % \setlength{\belowcaptionskip}{-10pt}
    \caption{Throughput Over Time During Reconfiguration}
    \label{fig:ev1-f1-timeline}
\end{figure}


==> figures/plots_code/experiments/Obsolete/EV1/f2.tex <==
\begin{figure}
    % \centering
	\begin{subfigure}{0.5\columnwidth}%
    	\centering
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev1-throughput-degradation.pdf}  
        \caption{Throughput Degradation During Reconfiguration}
        \label{fig:ev1_f2_a}
    \end{subfigure}%
    % \par\medskip
    \hfill
    \begin{subfigure}{0.5\columnwidth}%
    	\centering
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev1-unavailability-window.pdf}  
        \caption{Unavailability Window Duration}
        \label{fig:ev1_f2_b}
    \end{subfigure}%
    % \par\medskip 
    % \begin{subfigure}{0.8\columnwidth}%
    % 	\centering
    %     % \captionsetup{justification=centering}
      
    %     \includegraphics[width=\linewidth]{figures/plots/experiment/ev1-latency.pdf}  
    %     \caption{User Transaction Latency Distribution}
    %     \label{fig:ev1_f2_c}
    % \end{subfigure}%
    % \hfill

    % \begin{subfigure}{0.8\columnwidth}%
    % 	\centering
    %     % \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{figures/plots/experiment/ev-2-st-migr-txn-breakdown.pdf}  
    %     \caption{Reconfiguration Transaction Latency Breakdown }
    %     \label{fig:ev2_strategies_breakdown}
    % \end{subfigure}%
       % \par\medskip
    % \begin{subfigure}[b]{0.3\textwidth}%
    % 	\centering
    %     % \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{figures/plots/experiment/ev-2-migration-txn-latency.pdf}  

    %     \caption{Reconfiguration Transactions Latency Distribution}
    %     \label{fig:latency-distribution}
    % \end{subfigure}% 
    % \vspace{-.15in}
    % \setlength{\belowcaptionskip}{-10pt}
    \caption{Performance Analysis}
    \label{fig:ev1_f2}
\end{figure}

==> figures/plots_code/experiments/Obsolete/EV1/f3.tex <==
\begin{figure}
    % \centering

    % \begin{subfigure}{0.8\columnwidth}%
    	\centering
        % \captionsetup{justification=centering}
      
        \includegraphics[width=0.8\linewidth]{figures/plots/experiment/ev1-latency.pdf}  
        \caption{User Transaction Latency Distribution}
    % \end{subfigure}%
    % \hfill

    % \begin{subfigure}{0.8\columnwidth}%
    % 	\centering
    %     % \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{figures/plots/experiment/ev-2-st-migr-txn-breakdown.pdf}  
    %     \caption{Reconfiguration Transaction Latency Breakdown }
    %     \label{fig:ev2_strategies_breakdown}
    % \end{subfigure}%
       % \par\medskip
    % \begin{subfigure}[b]{0.3\textwidth}%
    % 	\centering
    %     % \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{figures/plots/experiment/ev-2-migration-txn-latency.pdf}  

    %     \caption{Reconfiguration Transactions Latency Distribution}
    %     \label{fig:latency-distribution}
    % \end{subfigure}% 
    % \vspace{-.15in}
    % \setlength{\belowcaptionskip}{-10pt}
    \label{fig:ev1_f2_c}
\end{figure}

==> figures/plots_code/experiments/Obsolete/EV1/t1.tex <==

\begin{table}[h]
    \centering
    % \caption{Performance Degradation Analysis}
     \setlength{\tabcolsep}{2pt}
    % \vspace{-3mm}
    \small
    \begin{tabular}{ l l l l l l }
    \toprule
    \textbf{Lines Of Code}&\textbf{\system}&\textbf{DynaMast}&\textbf{Albatross}&\textbf{Squall} \\ 
    \midrule
    Core & 243 & 395 & 666 & 233\\
    RPC & 101 & 130 & 143 & 100\\
    Total & 344 & 525 & 809 & 333\\
    \bottomrule
    \end{tabular}
    \vspace{3mm}
    % \setlength{\belowcaptionskip}{-10pt}
    \setlength{\abovecaptionskip}{-10pt}
    \caption{Implementation Complexity Comparison  --- \normalfont{"Core" is the core reconfiguration logic; "RPC" represents the RPC layer.} }
    
\label{tbl:ev1_t1}
\end{table}


% \begin{table}[h]
% \centering
% \begin{tabular}{|c|c|c|}
% \hline
% Column 1 & Column 2 & Column 3 \\ \hline
% Data 1   & Data 2   & Data 3   \\ 
% Data 4   & Data 5   & Data 6   \\ \hline
% \end{tabular}
% \caption{Example Table}
% \label{tbl:ev1_t1}
% \end{table}

==> figures/plots_code/experiments/Obsolete/EV2/f1.tex <==
\begin{figure*}[t]
	% \begin{subfigure}[b]{0.48\linewidth}%
        \centering
    \begin{subfigure}[t]{0.5\columnwidth}%h
    	\center
        \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev2-throughput-degradation.pdf}        
     \caption{Throughput Degradation for \system}
        \label{fig:ev2_f1_a}
    \end{subfigure}%
    \begin{subfigure}[t]{0.5\columnwidth}%
    	\center
        \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev2-reconfiguration-duration.pdf}        

     \caption{Reconfiguration Duration for \system}
        \label{fig:ev2_f1_b}
    \end{subfigure}%
    \begin{subfigure}[t]{0.5\columnwidth}%
    	\center
        \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev2-latency.pdf}        

     \caption{User Transaction Latency Distribution for \system}
        \label{fig:ev2_f1_c}
    \end{subfigure}%
    \begin{subfigure}[t]{0.5\columnwidth}%
    	\center
        \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev2-tradeoff.pdf}        

     \caption{Tradeoff Between Throughput Degradation and Duration}
        \label{fig:ev2_f1_d}
    \end{subfigure}%
    % \vspace{-.15in}
    \setlength{\belowcaptionskip}{-10pt}
    \caption{Performance Degradation vs. Reconfiguration Duration Across Concurrency Levels}
    \label{fig:ev2_f1}
\end{figure*}


==> figures/plots_code/experiments/Obsolete/EV2/obsolete/dur-perf-tradeoff.tex <==
\begin{figure}
    % \centering
	% \begin{subfigure}[b]{0.5\textwidth}%
        \begin{subfigure}{0.45\columnwidth}%
            \centering
            % \captionsetup{justification=centering}
            \includegraphics[width=\linewidth]{figures/plots/experiment/ev-2-st-strategy-tradeoff-hybrid-dur-throuput.pdf}  
            \caption{User Transactions Throughput Versus Reconfiguration Duration For Hybrid-Heat}
            \label{fig:ev2-tradeoff-hybrid-throughput}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.45\columnwidth}%
            \centering
            % \captionsetup{justification=centering}
            \includegraphics[width=\linewidth]{figures/plots/experiment/ev-2-st-strategy-tradeoff-hybrid-dur-latency.pdf}  
            \caption{User Transactions Latency Versus Reconfiguration Duration For Hybrid-Heat}
            \label{fig:ev2-tradeoff-hybrid-latency}
        \end{subfigure}%
        \par\medskip
        \begin{subfigure}{0.9\columnwidth}%
            \centering
            % \captionsetup{justification=centering}
            \includegraphics[width=0.8\linewidth]{figures/plots/experiment/ev-2-st-strategy-tradeoff-arithmean.pdf}  
            \caption{The Tradeoff Between Duration and Throughput Reconfiguration For Four Strategies}           
             \label{fig:ev2-tradeoff-four}
        \end{subfigure}%

    	% \centering
        % % \captionsetup{justification=centering}
        % \includegraphics[width=0.8\linewidth]{figures/plots/experiment/ev-2-st-strategy-tradeoff-arithmean.pdf}  

        \caption{Duration VS Performance Degradation}
        \label{fig:ev2-dur-perf-tradeoff}
    % \end{subfigure}%
    % \vspace{-.15in}
    % \setlength{\belowcaptionskip}{-10pt}
    % \caption{Performance under Contention}
    % \label{fig:contention_sknew}
\end{figure}



==> figures/plots_code/experiments/Obsolete/EV2/obsolete/fix-concurrency-compr-tbl.tex <==
\begin{table*}[t]
    \begin{center}
    \caption{Reconfiguration Cost for Different Strategies in \system}
    \label{tbl:fix-conc-tbl}
    \vspace{-3mm}
    \small
    \begin{tabular}{ l l l l l}
    \toprule
     \textbf{Indicators} & \textbf{Hybrid-Heat} & \textbf{Pre-Heat} & \textbf{Post-Heat} & \textbf{Naive}\\ 
    \midrule
    Reconfiguration Duration(s)& 19
        & 14 & 14 & >20 \\
    Throughput Degradation& 11.75\%
    & 16.36\% & 53.20\% & 57.27\% \\
    Avg Throughput During Reconfiguration(tps) & 4100.68
        & 4062.29 & 2132.36 & 1915.00 \\ 
    Avg Throughput Before Reconfiguration(tps) & 4646.90
        & 4857.05 & 4557.00 & 4482.25 \\ 

    Avg User Latency(ms)& 58.10
        & 55.69 & 66.07 & 80.56 \\
    P99 User Latency(ms)& 160.33
        & 129.06 & 335.65 & 368.45 \\
    P95 User Latency(ms)& 108.63 & 102.96 & 124.65 & 235.71 \\

    \bottomrule
    \end{tabular}
    \end{center}
    \end{table*}

==> figures/plots_code/experiments/Obsolete/EV2/obsolete/fix-strategy-compr-tbl.tex <==
\begin{table*}[t]
    \begin{center}
    \caption{Reconfiguration Cost for Hybrid-Heat Varying Concurrency}
    \label{tbl:fix-strategy-tbl}
    \vspace{-3mm}
    \small
    \begin{tabular}{ l l l l l l l  }
    \toprule
     \textbf{Indicators} & \textbf{1} & \textbf{2} & \textbf{4} & \textbf{8} & \textbf{16} & \textbf{32}\\ 
    \midrule
    Reconfiguration Duration(s)& 220
        & 114 & 59 & 31 & 19 & 21 \\
    Throughput Degradation& 4.21\%
    & 0.62\% & 1.18\% & 4.93\% & 11.75\% & 29.26\% \\
    Avg Throughput During Reconfiguration(tps) & 4523.43
        & 4656.25 & 4629.83 & 4447.52 & 4100.68 & 3324.05  \\ 
    Avg Throughput Before Reconfiguration(tps) & 4722.3
        & 4685.35 & 4685.15 & 4678.25 & 4646.9 & 4699.05  \\ 

    Avg User Latency(ms)& 56.22
        & 54.84 & 54.80 & 56.00 & 58.10 & 60.62\\
    P99 User Latency(ms)& 136.29
        & 125.68 & 125.75 & 125.84 & 160.33 & 143.61\\
    P95 User Latency(ms)& 104.91 & 99.99 & 100.86 & 101.97& 108.63& 106.26 \\

     \bottomrule
    \end{tabular}
    \end{center}
    \end{table*}

==> figures/plots_code/experiments/Obsolete/EV2/obsolete/hybrid-latency-thoughput-on-conc.tex <==
\begin{figure}
    % \centering
    \begin{subfigure}{0.4\columnwidth}%
    	\centering
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev-2-fix-strategy-latency-dist.pdf}  

        \caption{User Txn Latency Distribution}
        \label{fig:latency-distribution}
    \end{subfigure}%
    \begin{subfigure}{0.45\columnwidth}%
    	\centering
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev-2-st-migr-txn-breakdown-vary-conc.pdf}  
        \caption{Reconfiguration Txn Latency Breakdown}
        \label{fig:latency-distribution}
    \end{subfigure}%
    \par\medskip
	% \begin{subfigure}{0.45\columnwidth}%
    % 	\centering
    %     % \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{figures/plots/experiment/ev-2-st-strategy-tradeoff-hybrid-dur-throuput.pdf}  
    %     \caption{User Transactions Throughput Versus Reconfiguration Duration}
    %     \label{fig:latency-distribution}
    % \end{subfigure}%
    % \hfill
    % \begin{subfigure}{0.45\columnwidth}%
    % 	\centering
    %     % \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{figures/plots/experiment/ev-2-st-strategy-tradeoff-hybrid-dur-latency.pdf}  
    %     \caption{User Transactions Latency Versus Reconfiguration Duration}
    %     \label{fig:latency-breakdown}
    % \end{subfigure}%
       % \par\medskip
    % \begin{subfigure}[b]{0.3\textwidth}%
    % 	\centering
    %     % \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{figures/plots/experiment/ev-2-migration-txn-latency.pdf}  

    %     \caption{Reconfiguration Transactions Latency Distribution}
    %     \label{fig:latency-distribution}
    % \end{subfigure}% 
    % \vspace{-.15in}
    % \setlength{\belowcaptionskip}{-10pt}
    \caption{Performance Analysis for Hybrid-Heat Varying Concurrency}
    \label{fig:hybird-tradeoff-conc}
\end{figure}

==> figures/plots_code/experiments/Obsolete/EV2/obsolete/latency-analysis.tex <==
% \begin{figure*}[t!]
% 	% \begin{subfigure}[b]{0.48\linewidth}%
%         \centering

%     \begin{subfigure}[b]{0.3\linewidth}%
%     	% \center
%         % \captionsetup{justification=centering}
%         \includegraphics[width=\linewidth]{figures/plots/experiment/rampup.pdf}
%         \caption{Throughput for Ramp-Up Workload}
%         % \label{fig:rampup_compare}
%     \end{subfigure}%
%     \hfill

%     \begin{subfigure}[b]{0.3\linewidth}%
%     	% \center
%         % \captionsetup{justification=centering}
%         \includegraphics[width=\linewidth]{figures/plots/experiment/rampup_migr.pdf}  
%         \caption{Migration Transactions for Ramp-Up Workload}
%         % \label{fig:rampup_migr}
%     \end{subfigure}%
%     % \vspace{-.15in}
%     \setlength{\belowcaptionskip}{-5pt}
%     \caption{Performance on Ramp-Up Workload of \system versus On-premise Clusters}
%     \label{fig:lw_migr}
% \end{figure*}


\begin{figure*}[h]
	% \begin{subfigure}[b]{0.48\linewidth}%
        \centering

    \begin{subfigure}[b]{0.23\linewidth}%
    	\center
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev-2-st-hybrid-usertxn-latency.pdf}
        \caption{Hybrid-Heat}
        \label{fig:lsm_wf_put}
    \end{subfigure}%
    \begin{subfigure}[b]{0.23\linewidth}%
    	\center
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev-2-st-preheat-usertxn-latency.pdf}
     \caption{Pre-Heat}
        \label{fig:lsm_wf_get}
    \end{subfigure}%
    \begin{subfigure}[b]{0.23\linewidth}%
    	\center
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev-2-st-postheat-usertxn-latency.pdf}
     \caption{Post-Heat}
        \label{fig:lsm_wf_get}
    \end{subfigure}%
    \begin{subfigure}[b]{0.23\linewidth}%
    	\center
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev-2-st-noheat-usertxn-latency.pdf}
     \caption{Naive}
        \label{fig:lsm_wf_get}
    \end{subfigure}%
    % \vspace{-.15in}
    \setlength{\belowcaptionskip}{-10pt}
    \caption{Latency Distribution of User Transactions During Reconfiguration}
    \label{fig:latency_analysis}
\end{figure*}


==> figures/plots_code/experiments/Obsolete/EV2/obsolete/latency-breakdown.tex <==
\begin{figure}
    % \centering
	\begin{subfigure}{0.45\columnwidth}%
    	\centering
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev-2-st-strategy-usertxn-latency.pdf}  

        \caption{User Transaction Latency Distribution}
        \label{fig:ev2_strategies_user_latency_distribution}
    \end{subfigure}%
    \begin{subfigure}{0.45\columnwidth}%
    	\centering
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev-2-fix-conc-user-txn-throughput.pdf}  
        \caption{Average Throughput Degradation During Reconfiguration}
        \label{fig:ev2_strategies_avg_throughput}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.45\columnwidth}%
    	\centering
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev-2-fix-conc-reconfig-duration.pdf}  

        \caption{Reconfiguration Duration}
        \label{fig:ev2_strategies_duration}
    \end{subfigure}%
    \begin{subfigure}{0.45\columnwidth}%
    	\centering
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev-2-st-migr-txn-breakdown.pdf}  
        \caption{Reconfiguration Transaction Latency Breakdown }
        \label{fig:ev2_strategies_breakdown}
    \end{subfigure}%
       % \par\medskip
    % \begin{subfigure}[b]{0.3\textwidth}%
    % 	\centering
    %     % \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{figures/plots/experiment/ev-2-migration-txn-latency.pdf}  

    %     \caption{Reconfiguration Transactions Latency Distribution}
    %     \label{fig:latency-distribution}
    % \end{subfigure}% 
    % \vspace{-.15in}
    % \setlength{\belowcaptionskip}{-10pt}
    \caption{Reconfiguration Cost For Different Strategies}
    \label{fig:ev2_strategies_avg}
\end{figure}

==> figures/plots_code/experiments/Obsolete/EV2/obsolete/perfcmpr.tex <==



\begin{figure*}[t!]
	% \begin{subfigure}[b]{0.48\linewidth}%
        \centering
    \newcommand{\hybirdtl}{figures/plots/experiment/ev2-st-timeline-hybrid}
    \newcommand{\preheattl}{figures/plots/experiment/ev2-st-timeline-preheat}
    \newcommand{\postheattl}{figures/plots/experiment/ev2-st-timeline-postheat}
    \newcommand{\noheattl}{figures/plots/experiment/ev2-st-timeline-noheat}


    \begin{subfigure}[t]{0.2\linewidth}%
    	\center
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{\hybirdtl-1.pdf}  
        \includegraphics[width=\linewidth]{\hybirdtl-2.pdf}  
        \includegraphics[width=\linewidth]{\hybirdtl-4.pdf}  
        \includegraphics[width=\linewidth]{\hybirdtl-8.pdf}  
        \includegraphics[width=\linewidth]{\hybirdtl-16.pdf}  
        \includegraphics[width=\linewidth]{\hybirdtl-32.pdf}  
        \caption{Hybrid-Heat Reconfiguration}
        \label{fig:lsm_wf_put}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\linewidth}%
    	\center
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{\preheattl-1.pdf}  
        \includegraphics[width=\linewidth]{\preheattl-2.pdf}  
        \includegraphics[width=\linewidth]{\preheattl-4.pdf}  
        \includegraphics[width=\linewidth]{\preheattl-8.pdf}  
        \includegraphics[width=\linewidth]{\preheattl-16.pdf}  
        \includegraphics[width=\linewidth]{\preheattl-32.pdf}
     \caption{Pre-Heat Reconfiguration}
        \label{fig:lsm_wf_get}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\linewidth}%
    	\center
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{\postheattl-1.pdf}  
        \includegraphics[width=\linewidth]{\postheattl-2.pdf}  
        \includegraphics[width=\linewidth]{\postheattl-4.pdf}  
        \includegraphics[width=\linewidth]{\postheattl-8.pdf}  
        \includegraphics[width=\linewidth]{\postheattl-16.pdf}  
        \includegraphics[width=\linewidth]{\postheattl-32.pdf}
     \caption{Post-Heat Reconfiguration}
        \label{fig:lsm_wf_get}
    \end{subfigure}%
    \begin{subfigure}[t]{0.2\linewidth}%
    	\center
        % \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{\noheattl-1.pdf}  
        \includegraphics[width=\linewidth]{\noheattl-2.pdf}  
        \includegraphics[width=\linewidth]{\noheattl-4.pdf}  
        \includegraphics[width=\linewidth]{\noheattl-8.pdf}  
        \includegraphics[width=\linewidth]{\noheattl-16.pdf}  
        \includegraphics[width=\linewidth]{\noheattl-32.pdf}
     \caption{Naive Reconfiguration}
        \label{fig:lsm_wf_get}
    \end{subfigure}%
    % \vspace{-.15in}
    \setlength{\belowcaptionskip}{-10pt}
    \caption{Throughput Over Time for Different Strategies of Reconfiguration}
    \label{fig:ev2-perf-compr}
\end{figure*}


==> figures/plots_code/experiments/Obsolete/EV2/obsolete/strategy_perfcmpr.tex <==



\begin{figure}[h]
	% \begin{subfigure}[b]{0.48\linewidth}%
        \centering
    \newcommand{\hybirdtl}{figures/plots/experiment/ev2-st-timeline-hybrid}
    \newcommand{\preheattl}{figures/plots/experiment/ev2-st-timeline-preheat}
    \newcommand{\postheattl}{figures/plots/experiment/ev2-st-timeline-postheat}
    \newcommand{\noheattl}{figures/plots/experiment/ev2-st-timeline-noheat}

    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        % \captionsetup{justification=centering}
        % \includegraphics[width=\linewidth]{\hybirdtl-1.pdf}  
        % \includegraphics[width=\linewidth]{\hybirdtl-2.pdf}  
        % \includegraphics[width=\linewidth]{\hybirdtl-4.pdf}  
        % \includegraphics[width=\linewidth]{\hybirdtl-8.pdf}  
        \includegraphics[width=\linewidth]{\hybirdtl-16.pdf}  
        % \includegraphics[width=\linewidth]{\hybirdtl-32.pdf}  
        \caption{Hybrid-Heat}
        \label{fig:ev2-timeline-hybrid}
    \end{subfigure}%
    \par\medskip
    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        % \captionsetup{justification=centering}
        % \includegraphics[width=\linewidth]{\preheattl-1.pdf}  
        % \includegraphics[width=\linewidth]{\preheattl-2.pdf}  
        % \includegraphics[width=\linewidth]{\preheattl-4.pdf}  
        % \includegraphics[width=\linewidth]{\preheattl-8.pdf}  
        \includegraphics[width=\linewidth]{\preheattl-16.pdf}  
        % \includegraphics[width=\linewidth]{\preheattl-32.pdf}
     \caption{Pre-Heat}
        \label{fig:ev2-timeline-pre}
    \end{subfigure}%
    \par\medskip
    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        % \captionsetup{justification=centering}
        % \includegraphics[width=\linewidth]{\postheattl-1.pdf}  
        % \includegraphics[width=\linewidth]{\postheattl-2.pdf}  
        % \includegraphics[width=\linewidth]{\postheattl-4.pdf}  
        % \includegraphics[width=\linewidth]{\postheattl-8.pdf}  
        \includegraphics[width=\linewidth]{\postheattl-16.pdf}  
        % \includegraphics[width=\linewidth]{\postheattl-32.pdf}
     \caption{Post-Heat}
        \label{fig:ev2-timeline-post}
    \end{subfigure}%
    \par\medskip
    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        % \captionsetup{justification=centering}
        % \includegraphics[width=\linewidth]{\noheattl-1.pdf}  
        % \includegraphics[width=\linewidth]{\noheattl-2.pdf}  
        % \includegraphics[width=\linewidth]{\noheattl-4.pdf}  
        % \includegraphics[width=\linewidth]{\noheattl-8.pdf}  
        \includegraphics[width=\linewidth]{\noheattl-16.pdf}  
        % \includegraphics[width=\linewidth]{\noheattl-32.pdf}
     \caption{Naive}
        \label{fig:ev2-timeline-naive}
    \end{subfigure}%
    % \vspace{-.15in}
    \setlength{\belowcaptionskip}{-10pt}
    \caption{Throughput Over Time for Different Strategies of Reconfiguration}
    \label{fig:ev2-throughput-timeline-cmpr}
\end{figure}


==> figures/plots_code/experiments/Obsolete/EV3/f1.tex <==
\begin{figure}[t]
	% \begin{subfigure}[b]{0.48\linewidth}%
    \newcommand{\patha}{figures/plots/experiment/rampup}
    % \begin{subfigure}[b]{0.9\linewidth}%
    	\center
        \captionsetup{justification=centering}
        \includegraphics[width=0.9\linewidth]{figures/plots/experiment/ev3-scaleup.pdf}
        % \caption{Throughput Overtime}
        \label{fig:ev3_f1_a}
    % \end{subfigure}%
    % \par\medskip 
    % \begin{subfigure}[b]{0.5\linewidth}%
    % 	\center
    %     \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{figures/plots/experiment/ev3-scaleout-latency.pdf}
    %     \caption{Average Latency}
    %     \label{fig:ev3_f1_b}
    % \end{subfigure}%
    % \begin{subfigure}[b]{0.5\linewidth}%
    % 	\center
    %     \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{figures/plots/experiment/ev3-scaleout-cost.pdf}
    %     \caption{Total Costs}
    %     \label{fig:ev3_f1_c}
    % \end{subfigure}%


    % \begin{subfigure}[b]{0.8\linewidth}%
    % 	\center
    %     \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{figures/plots/experiment/rampup_migr.pdf}  
    %     \caption{Migration Transactions for Ramp-Up Workload}
    %     \label{fig:rampup_migr}
    % \end{subfigure}%
    \vspace{-.10in}
    \setlength{\belowcaptionskip}{-5pt}
    \caption{Acale-out scenario for \system.}
    % \caption{Performance on Scale-Out Workload of \system Versus On-premise Clusters}
    \label{fig:ev3_f1}
\end{figure}

==> figures/plots_code/experiments/Obsolete/EV3/f2.tex <==



\begin{figure}[h]
	% \begin{subfigure}[b]{0.48\linewidth}%
        \centering
    \newcommand{\marlintl}{figures/plots/experiment/ev3-LB-throughput-timeline-marlin}
    \newcommand{\dynamasttl}{figures/plots/experiment/ev3-LB-throughput-timeline-dynamast}
    \newcommand{\albtl}{figures/plots/experiment/ev3-LB-throughput-timeline-albatross}
    \newcommand{\postheattl}{figures/plots/experiment/ev3-LB-throughput-timeline-postheat}

    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        % \captionsetup{justification=centering}
        % \includegraphics[width=\linewidth]{\hybirdtl-1.pdf}  
        % \includegraphics[width=\linewidth]{\hybirdtl-2.pdf}  
        % \includegraphics[width=\linewidth]{\hybirdtl-4.pdf}  
        % \includegraphics[width=\linewidth]{\hybirdtl-8.pdf}  
        \includegraphics[width=\linewidth]{\marlintl.pdf}  
        % \includegraphics[width=\linewidth]{\hybirdtl-32.pdf}  
        % \caption{\system}
        \label{fig:ev3-f2-a}
    \end{subfigure}%
    % \vspace{-.05in}
    \par
    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        % \captionsetup{justification=centering}
        % \includegraphics[width=\linewidth]{\preheattl-1.pdf}  
        % \includegraphics[width=\linewidth]{\preheattl-2.pdf}  
        % \includegraphics[width=\linewidth]{\preheattl-4.pdf}  
        % \includegraphics[width=\linewidth]{\preheattl-8.pdf}  
        \includegraphics[width=\linewidth]{\dynamasttl.pdf}  
        % \includegraphics[width=\linewidth]{\preheattl-32.pdf}
    %  \caption{DynaMast}
     \label{fig:ev3-f2-b}
    \end{subfigure}%
    % \vspace{-.05in}
    \par
    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        % \captionsetup{justification=centering}
        % \includegraphics[width=\linewidth]{\postheattl-1.pdf}  
        % \includegraphics[width=\linewidth]{\postheattl-2.pdf}  
        % \includegraphics[width=\linewidth]{\postheattl-4.pdf}  
        % \includegraphics[width=\linewidth]{\postheattl-8.pdf}  
        \includegraphics[width=\linewidth]{\albtl.pdf}  

        % \includegroaphics[width=\linewidth]{\albatrosstl.pdf}  
        % \includegroaphics[width=\linewidth]{figures/plots/experiment/ev3-LB-throughput-timeline-albatross.pdf}  
        % \includegraphics[width=\linewidth]{\postheattl-32.pdf}
    %  \caption{Albatross}
     \label{fig:ev3-f2-c}
    \end{subfigure}%
    % \vspace{-.05in}
    \par
    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        % \captionsetup{justification=centering}
        % \includegraphics[width=\linewidth]{\noheattl-1.pdf}  
        % \includegraphics[width=\linewidth]{\noheattl-2.pdf}  
        % \includegraphics[width=\linewidth]{\noheattl-4.pdf}  
        % \includegraphics[width=\linewidth]{\noheattl-8.pdf}  
        \includegraphics[width=\linewidth]{\postheattl.pdf}  
        % \includegraphics[width=\linewidth]{\noheattl-32.pdf}
    %  \caption{Squall}
     \label{fig:ev3-f2-d}
    \end{subfigure}%
    % \vspace{-.05in}
    \vspace{-.15in}
    \setlength{\belowcaptionskip}{-6pt}
    \caption{Throughput Over Time for Load Balance Scenario}
    \label{fig:ev3_f2}
\end{figure}


==> figures/plots_code/experiments/Obsolete/EV3/f3.tex <==



\begin{figure}[h]
	% \begin{subfigure}[b]{0.48\linewidth}%
        \centering
    \newcommand{\marlintl}{figures/plots/experiment/ev3-SI-throughput-timeline-marlin}
    \newcommand{\dynamasttl}{figures/plots/experiment/ev3-SI-throughput-timeline-dynamast}
    \newcommand{\albtl}{figures/plots/experiment/ev3-SI-throughput-timeline-albatross}
    \newcommand{\postheattl}{figures/plots/experiment/ev3-SI-throughput-timeline-postheat}

    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        % \captionsetup{justification=centering}
        % \includegraphics[width=\linewidth]{\hybirdtl-1.pdf}  
        % \includegraphics[width=\linewidth]{\hybirdtl-2.pdf}  
        % \includegraphics[width=\linewidth]{\hybirdtl-4.pdf}  
        % \includegraphics[width=\linewidth]{\hybirdtl-8.pdf}  
        \includegraphics[width=\linewidth]{\marlintl.pdf}  
        % \includegraphics[width=\linewidth]{\hybirdtl-32.pdf}  
        % \caption{\system}

        \label{fig:ev3-f2-a}
    \end{subfigure}%
    \vspace{-.05in}

    \par\medskip
    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        % \captionsetup{justification=centering}
        % \includegraphics[width=\linewidth]{\preheattl-1.pdf}  
        % \includegraphics[width=\linewidth]{\preheattl-2.pdf}  
        % \includegraphics[width=\linewidth]{\preheattl-4.pdf}  
        % \includegraphics[width=\linewidth]{\preheattl-8.pdf}  
        \includegraphics[width=\linewidth]{\dynamasttl.pdf}  
        % \includegraphics[width=\linewidth]{\preheattl-32.pdf}
    %  \caption{DynaMast}
     \label{fig:ev3-f2-b}
    \end{subfigure}%
    \vspace{-.05in}

    \par\medskip
    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        % \captionsetup{justification=centering}
        % \includegraphics[width=\linewidth]{\postheattl-1.pdf}  
        % \includegraphics[width=\linewidth]{\postheattl-2.pdf}  
        % \includegraphics[width=\linewidth]{\postheattl-4.pdf}  
        % \includegraphics[width=\linewidth]{\postheattl-8.pdf}  
        \includegraphics[width=\linewidth]{\albtl.pdf}  

        % \includegroaphics[width=\linewidth]{\albatrosstl.pdf}  
        % \includegroaphics[width=\linewidth]{figures/plots/experiment/ev3-LB-throughput-timeline-albatross.pdf}  
        % \includegraphics[width=\linewidth]{\postheattl-32.pdf}
    %  \caption{Albatross}
     \label{fig:ev3-f2-c}
    \end{subfigure}%
    \vspace{-.05in}

    \par\medskip
    \begin{subfigure}[t]{0.95\columnwidth}%
    	\center
        % \captionsetup{justification=centering}
        % \includegraphics[width=\linewidth]{\noheattl-1.pdf}  
        % \includegraphics[width=\linewidth]{\noheattl-2.pdf}  
        % \includegraphics[width=\linewidth]{\noheattl-4.pdf}  
        % \includegraphics[width=\linewidth]{\noheattl-8.pdf}  
        \includegraphics[width=\linewidth]{\postheattl.pdf}  
        \vspace{-.4in}
        % \includegraphics[width=\linewidth]{\noheattl-32.pdf}
    %  \caption{Squall}
     \label{fig:ev3-f2-d}
    \end{subfigure}%
    % \vspace{-.15in}
    % \setlength{\belowcaptionskip}{-10pt}
    \caption{Throughput Over Time for Scale In Scenario}
    \label{fig:ev3_f3}
\end{figure}


==> figures/plots_code/experiments/Obsolete/EV3/fault-tolerance.tex <==
\begin{figure}
	% \begin{subfigure}[b]{0.48\linewidth}%
    \newcommand{\ftpath}{figures/plots/experiment/ev3-ft-timeline}

    \center
    \captionsetup{justification=centering}
    \includegraphics[width=\linewidth]{\ftpath.pdf}
    % \begin{subfigure}[b]{0.7\linewidth}%
    % 	\center
    %     \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{\ftpath-1.pdf}
    %     \caption{1}
    %     % \label{fig:rampup_compare}
    % \end{subfigure}%
    % \par\medskip
    % \begin{subfigure}[b]{0.7\linewidth}%
    % 	\center
    %     \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{\ftpath-4.pdf}
    %     \caption{4}
    %     % \label{fig:rampup_migr}
    % \end{subfigure}%
    % \par\medskip
    % \begin{subfigure}[b]{0.7\linewidth}%
    % 	\center
    %     \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{\ftpath-8.pdf}
    %     \caption{8}
    %     % \label{fig:rampup_migr}
    % \end{subfigure}%
    % \par\medskip
    % \begin{subfigure}[b]{0.7\linewidth}%
    % 	\center
    %     \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{\ftpath-16.pdf}
    %     \caption{16}
    %     % \label{fig:rampup_migr}
    % \end{subfigure}%
    % % \vspace{-.15in}
    \setlength{\belowcaptionskip}{-5pt}
    \caption{Throughput Over Time for Node Failure Scenario}
    \label{fig:fault-tolerance}
\end{figure}

==> figures/plots_code/experiments/Obsolete/EV3/load-balance.tex <==
\begin{figure}
	% \begin{subfigure}[b]{0.48\linewidth}%
    \newcommand{\lbpath}{figures/plots/experiment/ev3-lb-timeline}
    \center
    \captionsetup{justification=centering}
    \includegraphics[width=\linewidth]{\lbpath.pdf}
    % \begin{subfigure}[b]{0.7\linewidth}%
    % 	\center
    %     \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{\lbpath-1.pdf}
    %     \caption{1}
    %     \label{fig:rampup_compare}
    % \end{subfigure}%
    % \par\medskip
    % \begin{subfigure}[b]{0.7\linewidth}%
    % 	\center
    %     \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{\lbpath-4.pdf}
    %     \caption{4}
    %     \label{fig:rampup_migr}
    % \end{subfigure}%
    % \par\medskip
    % \begin{subfigure}[b]{0.7\linewidth}%
    % 	\center
    %     \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{\lbpath-8.pdf}
    %     \caption{8}
    %     \label{fig:rampup_migr}
    % \end{subfigure}%
    % \par\medskip
    % \begin{subfigure}[b]{0.7\linewidth}%
    % 	\center
    %     \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{\lbpath-16.pdf}
    %     \caption{16}
    %     \label{fig:rampup_migr}
    % \end{subfigure}%
    % \vspace{-.15in}
    \setlength{\belowcaptionskip}{-5pt}
    \caption{Throughput Over Time for Load Balance Scenario}
    \label{fig:loadbalance-timeline}
\end{figure}

==> figures/plots_code/experiments/Obsolete/EV3/scale-in.tex <==
\begin{figure}
	% \begin{subfigure}[b]{0.48\linewidth}%
    \newcommand{\scaleinpath}{figures/plots/experiment/ev3-si-timeline}
    \center
    \captionsetup{justification=centering}
    \includegraphics[width=\linewidth]{\scaleinpath.pdf}
    % \begin{subfigure}[b]{0.7\linewidth}%
    % 	\center
    %     \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{\scaleinpath-1.pdf}
    %     \caption{1}
    %     \label{fig:rampup_compare}
    % \end{subfigure}%
    % \par\medskip
    % \begin{subfigure}[b]{0.7\linewidth}%
    % 	\center
    %     \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{\scaleinpath-4.pdf}
    %     \caption{4}
    %     \label{fig:rampup_migr}
    % \end{subfigure}%
    % \par\medskip
    % \begin{subfigure}[b]{0.7\linewidth}%
    % 	\center
    %     \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{\scaleinpath-8.pdf}
    %     \caption{8}
    %     \label{fig:rampup_migr}
    % \end{subfigure}%
    % \par\medskip
    % \begin{subfigure}[b]{0.7\linewidth}%
    % 	\center
    %     \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{\scaleinpath-16.pdf}
    %     \caption{16}
    %     \label{fig:rampup_migr}
    % \end{subfigure}%

    % \vspace{-.15in}
    \setlength{\belowcaptionskip}{-5pt}
    \caption{Throughput Over Time for Scale In Scenario}
    \label{fig:scalein-timeline}
\end{figure}

==> figures/plots_code/experiments/Obsolete/lw-reconf/lightweight.tex <==
\begin{figure*}[t]
	% \begin{subfigure}[b]{0.48\linewidth}%
        \centering
    \begin{subfigure}[t]{0.5\columnwidth}%h
    	\center
        \captionsetup{justification=centering}
        % \includegraphics[width=\linewidth]{figures/plots/experiment/ev-1-usertxn-latency.pdf}        
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev-1-usertxn-throughput.pdf}        
     \caption{Average Throughut of User Transactions}
        \label{fig:lw_migr_user_throughput}
    \end{subfigure}%
    \begin{subfigure}[t]{0.5\columnwidth}%
    	\center
        \captionsetup{justification=centering}
        % \includegraphics[width=\linewidth]{figures/plots/experiment/ev-1-usertxn-latency.pdf}        
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev-1-st-lightweight-usertxn-latency.pdf}        
     \caption{Latency Distribution of User Transactions}
        \label{fig:lw_migr_user_latency}
    \end{subfigure}%
    \begin{subfigure}[t]{0.5\columnwidth}%
    	\center
        \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev-1-usertxn-abort-ratio.pdf}        
     \caption{Abort Ratio of User Transactions}
        \label{fig:lw_migr_abort}
    \end{subfigure}%
    \begin{subfigure}[t]{0.5\columnwidth}%
    	\center
        \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{figures/plots/experiment/ev-1-migration-txn-latency.pdf}
        \caption{Latency Distribution of Reconfiguration Transactions}
        \label{fig:lw_migr_reconf_latency}
    \end{subfigure}%
    % \vspace{-.15in}
    \setlength{\belowcaptionskip}{-10pt}
    \caption{Overhead Of Naive Reconfiguration(Varying Reconfiguration Rate)}
    \label{fig:lw_migr}
\end{figure*}


==> figures/plots_code/experiments/Obsolete/rampup/rampup.tex <==
\begin{figure}[t]
	% \begin{subfigure}[b]{0.48\linewidth}%
    \newcommand{\patha}{figures/plots/experiment/rampup}
    \begin{subfigure}[b]{0.9\linewidth}%
    	\center
        \captionsetup{justification=centering}
        \includegraphics[width=\linewidth]{\patha.pdf}
        \caption{Throughput for Scale-Out Workload}
        \label{fig:rampup_compare}
    \end{subfigure}%

    % \begin{subfigure}[b]{0.8\linewidth}%
    % 	\center
    %     \captionsetup{justification=centering}
    %     \includegraphics[width=\linewidth]{figures/plots/experiment/rampup_migr.pdf}  
    %     \caption{Migration Transactions for Ramp-Up Workload}
    %     \label{fig:rampup_migr}
    % \end{subfigure}%
    % \vspace{-.15in}
    \setlength{\belowcaptionskip}{-5pt}
    \caption{Performance on Scale-Out Workload of \system Versus On-premise Clusters}
    \label{fig:rampup}
\end{figure}

==> figures/plots_code/experiments/Obsolete/scaleout/so_timeline.tex <==
\begin{figure}
    % \centering
	% \begin{subfigure}[b]{0.5\textwidth}%
    	\centering
        % \captionsetup{justification=centering}
        \includegraphics[width=0.8\linewidth]{figures/plots/experiment/so_timeline.pdf}  

        \caption{Performance in Scale Out Scenario. The Bars Show Throughput.}
        \label{fig:so_timeline}
    % \end{subfigure}%
    % \vspace{-.15in}
    % \setlength{\belowcaptionskip}{-10pt}
    % \caption{Performance under Contention}
    % \label{fig:contention_sknew}
\end{figure}

==> sections/5_correctness.tex <==
\clearpage
\section{Proof of Correctness}
\label{sec:correctness}

\gzh{we have not presented the full picture of how \system works upon migrations (previous subsec was just about the txn mechanisms) nor any invariants we define \system to maintain. This subsec goes straight into a proof and I'm kind of lost about what needs to be proved.}
\wjh{update}
The two consistency guarantees (\secref{subsubsec:systable}) on system tables are crucial for correctness. In this section, we prove that they are properly enforced in  \system. 
%This section proves that ensuring correct cluster management. They form the basis of the integrity constraint for partitioned user tables, ensuring that each data record is owned by only one node at any time. We summarize them into \cref{theo:gtbl} and provide the proof below.
We make the following assumptions on the initial state of the system:
\begin{hypothesis}
\label{hyp:initial}
After data loading, the system is in a consistent initial state where \utbl is correctly partitioned by the primary key and the two consistency guarantees on system tables are satisfied. %ACID is guaranteed for all transactions, which is provided by classical protocols(e.g., 2PL, 2PC).
\end{hypothesis}

\begin{theorem}
    \label{theo:gtbl}
        \textbf{System Table Consistency.} 
        \mtbl is always consistent across all compute nodes in the cluster. 
        The contents of a local \gtbl may diverge slightly from the ground truth, but the local \gtbl must have \textit{\textbf{identical content}} as the ground truth regarding granules mapped the current node.
        % From \gtbl, each compute node must see all and only those granules that it owns. 
\end{theorem}
\vspace{-.2in}

\begin{proof}
We prove the theorem by induction. Initially, the theorem holds as per \cref{hyp:initial}.
We will show that %\textit{Induction step:} Assuming \gtbl and \mtbl adhere to the theorem before a transaction, we demonstrate 
the theorem continues to hold after the execution of transactions.

\textbf{Consistency for \mtbl.} User transactions and \textit{MigrationTxn} do not modify \mtbl and do not affect its consistency. \textit{AddNodeTxn} commits its commits to \mtbl in all compute nodes through the %, with a coordinator committing on \syslog. The 
distributed atomic commit protocol. % ensures consistency, regardless of failures. 
Therefore, all nodes will see a consistent view of \mtbl after the transaction. For \textit{DeleteNodeTxn}, if it is triggered to delete an alive node, the theorem holds for the same reason as \textit{AddNodeTxn}. If it is triggered to delete a failed node, the coordinator will commit to the \datalog of the failed node on behalf and other nodes. % in \mtbl will commit by themselves (see \secref{subsec:failure}). 
Therefore, every active node in \mtbl (and  the failed node's log as well) 
will see a consistent view of \mtbl. %decision for the node deletion after the transaction.

\textbf{Consistency for \gtbl.} The theorem holds for user transactions, \textit{AddNodeTxn}, and \textit{DeleteNodeTxn} since they do not modify \gtbl. For a committed \textit{MigrationTxn}, the coordinator writes the ownership change to \syslog, which holds the ground truth. % Therefore, the granules mapped to the source node and the destination node in the ground truth are changed. 
As the transaction is committed on both the source and destination nodes, their local \gtbl will reflect these updates. Therefore, the local \gtbl of the source and the destination nodes have identical content as the ground truth regarding the migrating granule. Since the modification does not involve any granule owned by other nodes, the theorem holds for every node. 
%\textit{Conclusion:} The theorem holds initially and remains valid through any sequence of transactions.
\end{proof}

